Multi-Designated Detector Watermarking for Language Models

In this paper, we initiate the study of \emph{multi-designated detector watermarking (MDDW)} for large language models (LLMs). This technique allows model providers to generate watermarked outputs from LLMs with two key properties: (i) only specific, possibly multiple, designated detectors can identify the watermarks, and (ii) there is no perceptible degradation in the output quality for ordinary users. We formalize the security definitions for MDDW and present a framework for constructing MDDW for any LLM using multi-designated verifier signatures (MDVS). Recognizing the significant economic value of LLM outputs, we introduce claimability as an optional security feature for MDDW, enabling model providers to assert ownership of LLM outputs within designated-detector settings. To support claimable MDDW, we propose a generic transformation converting any MDVS to a claimable MDVS. Our implementation of the MDDW scheme highlights its advanced functionalities and flexibility over existing methods, with satisfactory performance metrics.

==> 4pseudoMDVS.tex <==
% \clearpage
\section{A construction of pseudorandom MDVS}
\label{sec:concrete_mdvs}
Although numerous MDVS schemes have been proposed in the literature  \cite{chow2008multi,au2014strong,damgaard2020stronger,maurer2022multi,chakraborty2023deniable}, these schemes  do not exhibit pseudorandomness. 
The reason is that these MDVS schemes provide some partial  public verification  (via NIZK proof or ring signature) for ordinary users, thus undermining the pseudorandom properties.

%Now, we introduce a generic transform from any MDVS schemes without pseudorandomness to pseudorandom MDVS schemes. For simplicity, in the following we use PMDVS to denote pseudorandom MDVW schemes, distinguishing those without pseudorandomness.

We now present a generic transformation that converts any MDVS scheme lacking pseudorandomness into a pseudorandom MDVS scheme (PMDVS). For ease of discussion, we will refer to the latter as PMDVS to distinguish it from its non-pseudorandom counterparts.

\input{PKEctpr.tex}

\subsection{PMDVS construction}

\noindent \underline{\textbf{A generic transformation.}}
% \label{sec:gen_trans}
% As discussed in the aforementioned section, some DVS schemes (e.g., \cite{li2007designated,lipmaa2005designated}) are not pseudorandom, because some DVS schemes provide part verification (e.g., NIZK proof) for the common users. Here, we provide a generic transform from any DVS to pseudorandom DVS.
% 
The main idea is simple. To generate a PMDVS signature, the signer firstly generates a MDVS signature, and then encrypts it  via a PKE scheme, using the public keys of the designated verifiers. 
%provide pseudorandomness, the signer further encrypts the MDVS signature via an asymmetric encryption scheme, using the public key of the designated verifiers. 
Note that as long as the PKE scheme has ciphertext pseudorandomness, then the obtained ciphertexts constitute a pseudorandom signature,  and only the designated verifiers  could decrypt the ciphertexts to recover the underlying MDVS  signature, and then verify it. %. For instance, there are some encryption schemes working over the multiplicative group of integers modulo a prime $p$, e.g., ElGamal encryption \cite{elgamal1985public}, and these schemes are appropriate. In \cite{moller2004public}, authors also presents a practical public-key encryption scheme that offers security under adaptive chosen-ciphertext attack (CCA) and has pseudorandom ciphertexts.
%In this way, only the designated verifiers could decrypt the ciphertext to obtain the signature, and then verify it. 

Now we turn to the details. 

Let $\pke=(\pke.\setup,\pke.\kg,\pke.\enc,\pke.\dec)$ be a PKE scheme, % has ciphertext pasudorandomness, %  as recalled in Sec. \ref{sec:pre_pke}. 
and  $\mdvs=(\mdvs.\setup,\mdvs.\skg,\mdvs.\vkg,$ $\mdvs.\sign,\mdvs.\verify)$ be a MDVS scheme whose signature space is the same as the message space of $\pke$. % recalled in Sec. \ref{sec:MDVS_definition}. 
%We require that the message space of $\pke$ is the same as the signature space of $\mdvs$. 

As mentioned above, all verifiers in some set $S$ share a pair of public key and secret key of the PKE scheme. It can be achieved by kinds of methods. For example, the key pair is generated by a trusted third party or is generated via secure MPS, and then the key pair is shared via the private communication channels or even delivered off-line. We omit the details here. To ease the description of the key generation of PKE in the PMDVS, we define following algorithms (or protocols), which are used as a black-box:
\begin{myitemize}
    \item $\pkset(\pp,S) \rightarrow pk$: On input the public parameter $\pp$ and a set $S \subseteq [n]$, it returns a public key $pk$ of the PKE scheme for the set $S$.
    \item $\skset(\pp,S)  \rightarrow sk$: On input the public parameter $\pp$ and a set $S \subseteq [n]$, it outputs the corresponding secret key $sk$ for the $pk \leftarrow \pkset(\pp,S)$, and delivers $sk$ to the verifiers in $S$ \emph{privately}. The verifiers not in $S$ cannot receive $sk$.
\end{myitemize}

We assume that the key $pk$ output by $\pkset(\pp,S)$ and $sk$ output by $\skset(\pp,S)$ for the set $S$ are identical to $(pk,sk)$ output by $\pke.\kg$.
% To ease our description, we introduce an algorithm $\kgset(\pp)$ which is run by all the verifiers in some set $S \subseteq [n]$. It takes as input the public parameter $\pp$ output by the setup algorithm $\setup$ of some IND-secure PKE scheme with pseudorandom ciphertext, i.e., $\pp \leftarrow \pke.\setup(1^{\lambda})$, and then it invokes key generation algorithm $(pk,sk) \leftarrow \pke.\kg(\pp)$. Finally, it delivers the corresponding key pair $(pk,sk)$ to the verifiers in $S$ \emph{privately}.

Then, we construct a generic transform from any MDVS to PMDVS in Fig. \ref{fig:algo_topmdvs}.

% Note that all verifiers share a pair of public key and secret key of the PKE scheme. The keys can be shared via the secret communication channels or via secure MPC. Here, we omit the details, and define a following function, which is used as a black-box:
% \begin{itemize}
%     \item $\kgset(\pp,S)$: On input the public parameter $\pp$ of a PKE scheme and a set $S \subseteq [n]$, it  returns a public key $pk$ for the PKE scheme and delivers the corresponding secret key $sk$ to the users in $S$ \emph{privately}.
%     \item $\pkset(\pp,S)$: On input the public parameter $\pp$ of a PKE scheme and a set $S \subseteq [n]$, it invokes  returns a public key $pk$ for the PKE scheme and delivers the corresponding secret key $sk$ to the users in $S$ \emph{privately}.
% \end{itemize}
% \begin{algorithm}
%     \caption{$\topdvs(\pp,\ssk,\vpk,m)$ }
%     \label{algo:topdvs}
%     $\setup(1^{\lambda})$:\\
%     $(\vpk^{\mdvs},\vpk^{\pke})\leftarrow \vpk$\\
%     $\sigma' \leftarrow \mdvs.\sign(\pp,\ssk,\vpk^{\mdvs},m)$\\
%     \Return $\sigma:= c \leftarrow \pke.\enc(\vpk^{\pke},\sigma')$
%     % $\sigma := c$
%     \end{algorithm}

    \begin{figure}[!h]
        % \scriptsize
        \small
        % \vspace{-12pt}
        \centering
        % \hspace{-0.07\textwidth}
        %\begin{tabular}[c]{|p{18cm}|}\hline
            \fbox{
                \begin{minipage}
                    % [h][5.2cm]
                    [t]{0.89\textwidth}{
                    \underline{$\setup(1^{\lambda})$}:\\
                    Return $\pp := (\pp_{\mdvs} \leftarrow \mdvs.\setup(1^{\lambda})$, $\pp_{\pke} \leftarrow \pke.\setup(1^{\lambda}) )$\\
                    % Choose a PRG $\prg$: $\G \rightarrow \{0,1\}^{2*|\G|+5*|\Z|}$\\
                    % Return $\pp=(\pp_{\mdvs},\pp_{\pke})$\\

                    \underline{$\skg(\pp)$}:\\
                                    Return $(\spk,\ssk) \leftarrow \mdvs.\skg(\pp_{\mdvs})$\\
    
                                    \underline{$\vkg(\pp)$}:\\
                                    % $(\vpk^{\mdvs},\vsk^{\mdvs}) \leftarrow \mdvs.\vkg(\pp_{\mdvs})$\\
                                    Return $(\vsk,\vpk)\leftarrow \mdvs.\vkg(\pp_{\mdvs})$\\
                                    % $(\vpk^{\pke},\vsk^{\pke}) \leftarrow \kgset(\pp_{\pke})$\hfill $//$ Verifiers in $S$ share the keys\\
                                    % Return $(\vsk=(\vsk^{\mdvs},\vsk^{\pke}),\vpk=(\vpk^{\mdvs},\vpk^{\pke}))$\\
    
                                    \underline{$\sign(\pp,\ssk_i,(\vpk_j)_{j \in S},m)$}: \hfill $\sslash S$ contains the identities of all verifiers.\\
                                    % For $j\in S$: $(\vpk_j^{\mdvs},\vpk^{\pke})\leftarrow \vpk_j$\\
                                    % $\hat{\sigma} \leftarrow \mdvs.\sign(\pp_{\mdvs},\ssk_i,(\vpk_j^{\mdvs})_{j\in S},m)$\\
                                    % Return $\sigma:= (c \leftarrow \pke.\enc(\pp_{\pke},\vpk^{\pke},\hat{\sigma}))$\\
                                    $pk \leftarrow \pkset(\pp_{\pke},S)$,
                                    $\hat{\sigma} \leftarrow \mdvs.\sign(\pp_{\mdvs},\ssk_i,(\vpk_j)_{j\in S},m)$\\
                                    Return $\sigma:= (c \leftarrow \pke.\enc(\pp_{\pke},pk,\hat{\sigma}))$\\
    
                    \underline{$\verify(\pp,\spk_i,\vsk_{j'},(\vpk_j)_{j\in S},m,\sigma)$}:\hfill$\sslash j'\in S$\\
                                        % For $j\in S$: $(\vsk_j^{\mdvs},\vsk^{\pke})\leftarrow \vsk_j$, $(\vpk_j^{\mdvs},\vpk^{\pke})\leftarrow \vpk_j$\\
                                        % $\hat{\sigma} \leftarrow \pke.\dec(\pp_{\pke},\vsk^{\pke},c=\sigma)$\\
                                        % Return $b \leftarrow \mdvs.\verify(\pp_{\mdvs},\spk_i,\vsk_{j'}^{\mdvs}, (\vpk_j^{\mdvs})_{j\in S},\hat{\sigma})$
                                        % % Return $b$
                                        $sk \leftarrow \skset(\pp_{\pke},S)$,
                                        $\hat{\sigma} \leftarrow \pke.\dec(\pp_{\pke},sk,c=\sigma)$\\
                                        Return $b \leftarrow \mdvs.\verify(\pp_{\mdvs},\spk_i,\vsk_{j'}, (\vpk_j)_{j\in S},\hat{\sigma})$
    
                        % \begin{minipage}
                        %     % 	% [h][5.2cm]
                        %         [t]{0.45\textwidth}{
                        %             \underline{$\skg(\pp)$}:\\
                        %             Return $(\ssk,\spk) \leftarrow \mdvs.\skg(\pp_{\mdvs})$\\
    
                        %             \underline{$\vkg(\pp)$}:\\
                        %             $(\vsk^{\pke},\vpk^{\pke}) \leftarrow \pke.\vkg(\pp_{\pke})$\\
                        %             $(\vsk^{\mdvs},\vpk^{\mdvs}) \leftarrow \mdvs.\vkg(\pp_{\mdvs})$\\
                        %             Return $(\vsk=(\vsk^{\mdvs},\vsk^{\pke}),\vpk=(\vpk^{\mdvs},\vpk^{\pke}))$\\
    
                        %             \underline{$\sign(\pp,\ssk,\vpk,m)$}:\\
                        %             $(\vpk^{\mdvs},\vpk^{\pke})\leftarrow \vpk$\\
                        %             $\sigma' \leftarrow \mdvs.\sign(\pp,\ssk,\vpk^{\mdvs},m)$\\
                        %             Return $\sigma:= c \leftarrow \pke.\enc(\vpk^{\pke},\sigma')$
                        %          }
                        %      \end{minipage}	
                        %      \hspace{0.01\textwidth}
                        %      \begin{minipage}
                        %         % 	% [h][5.2cm]
                        %             [t]{0.45\textwidth}{
                        %                 \underline{$\verify(\pp,\spk,\vsk,m,\sigma)$}:\\
                        %                 $(\vsk^{\mdvs},\vsk^{\pke})\leftarrow \vsk$\\
                        %                 $\sigma' \leftarrow \pke.\dec(\pp_{\pke},c=\sigma,\vsk^{\pke})$\\
                        %                 $b \leftarrow \mdvs.\verify(\pp_{\mdvs},\vsk^{\mdvs},\sigma')$\\
                        %                 Return $b$
    
                        %                 % \underline{$\forge(\pp,\spk,\vsk,m)$}:\\
                        %                 % $r\leftarrow \{0,1\}^*$, $h \leftarrow \hashf_0(m,r)$\\
                        %                 % $s \leftarrow \hashf_1(e(\spk,h^{\vsk}))$\\
                        %                 % Return $\sigma := (r,s)$
                        %              }
                        %          \end{minipage}	
                     }
                 \end{minipage}
                %	\vrule
                %  \hspace{0.01\textwidth}
                %  \begin{minipage}
                % % 	% [h][5.2cm]
                % 	[t]{0.31\textwidth}{
                %         \underline{$\sign(\pp,\ssk,\vpk,m)$}:\\
                %         $r\leftarrow \{0,1\}^*$, $h \leftarrow \hashf_0(m,r)$\\
                %         $s \leftarrow \hashf_1(e(\vpk,h^{\ssk}))$\\
                %         Return $\sigma := (r,s)$\\
    
                %         \underline{$\forge(\pp,\spk,\vsk,m)$}:\\
                %         $r\leftarrow \{0,1\}^*$, $h \leftarrow \hashf_0(m,r)$\\
                %         $s \leftarrow \hashf_1(e(\spk,h^{\vsk}))$\\
                %         Return $\sigma := (r,s)$\\
    
                %         \underline{$\verify(\pp,\spk,\vsk,m,\sigma)$}:\\
                %         $(r,s) \leftarrow \sigma$, $h \leftarrow \hashf_0(m,r)$\\
                %         If $(s \neq \hashf_1(e(\spk,h^{\vsk})))$:\\
                %         $~~~~$Return $0$\\
                %         Return $1$
                %  	}
                %  \end{minipage}	
    }	
        % \setlength{\abovecaptionskip}{2pt}
        % \setlength{\belowcaptionskip}{-12pt}
        \captionsetup{justification=centering}
        \caption{PMDVS from any DVS}
        \label{fig:algo_topmdvs}
    \end{figure}

% Note that for the algorithms $\sign$ and $\verify$ in Fig. \ref{fig:algo_topmdvs}, it is required that all verifiers in $S$ should share the same public key and secret key of the $\pke$. If not, then these algorithms would abort.

The correctness of $\pmdvs$ is trivially guaranteed by the correctness of the underlying encryption scheme $\pke$ and the DVS scheme $\mdvs$. We omit the analysis of correctness here.

\noindent \underline{\textbf{Security analysis.}} We have the following theorem.
\begin{theorem}
    If the PKE scheme $\pke$ is secure and has ciphertext pseudorandomness, the MDVS scheme $\mdvs$ is consistent and existentially unforgeable, the pseudorandom MDVS constructed above is consistent, existential unforgeable and pseudorandom.
    \label{theo:topmdvs}
\end{theorem}

In the following, we prove Theorem \ref{theo:topmdvs}. 

\noindent \underline{\emph{Consistency.}} Assume that there exists an adversary $\A$ can win the consistency game of $\pmdvs$ with non-negligible probability. Then, we construct another adversary $\B$ to break the consistency game of $\mdvs$.

The construction is as follows.

Once $\B$ receives $\pp_{\mdvs}$ from the challenger of consistency game of $\mdvs$, $\B$ runs $\pp_{\pke} \leftarrow \pke.\setup(1^{\lambda})$ and forwards $\pp=(\pp_{\mdvs},\pp_{\pke})$ to $\A$. 
% it  and $(\vpk^{\pke},\vsk^{\pke}) \leftarrow \pke.\kg(\pp_{\pke})$, and then sets $\pp=(\pp_{\mdvs},\pp_{\pke})$, $\vpk=(\vpk^{\mdvs},\vpk^{\pke})$. After that, it forwards $\A$ the tuple $(\pp,\spk,\vpk)$.
% $\B$ also runs $(\vpk^{\pke},\vsk^{\pke}) \leftarrow \pke.\kg(\pp_{\pke})$, such that all verifiers would get the same $(\vpk^{\pke},\vsk^{\pke})$.

Then $\B$ answers the queries from $\A$.
\begin{itemize}
    \item $\mathcal{O}_{SK}(i)$: When $\A$ makes $\mathcal{O}_{SK}$ queries on $i$, $\B$ firstly forwards the queries to the challenger of consistency game of $\mdvs$. After receiving the reply $(\spk_i,\ssk_i)$ from the challenger, $\B$ forwards $(\spk_i,\ssk_i)$ to $\A$.
    \item $\mathcal{O}_{VK}(j)$: When $\A$ makes $\mathcal{O}_{VK}$ queries on $j$, $\B$ firstly forwards the queries to the challenger of consistency game of $\mdvs$. After receiving the reply $(\vpk_j,\vsk_j)$ from the challenger, $\B$ forwards $(\vpk_j,\vsk_j)$
    %  $(\vpk_j = (\vpk_j^{\mdvs},\vpk^{\pke}),\vsk_j=(\vsk_j^{\mdvs},\vsk^{\pke}))$ 
     to $\A$.
    \item $\mathcal{O}_{SPK}(i)$: When $\A$ makes $\mathcal{O}_{SPK}$ queries on $i$, $\B$ firstly forwards the queries to the challenger of consistency game of $\mdvs$. After receiving the reply $\spk_i$ from the challenger, $\B$ forwards $\spk_i$ to $\A$.
    \item $\mathcal{O}_{VPK}(j)$: When $\A$ makes $\mathcal{O}_{VPK}$ queries on $j$, $\B$ firstly forwards the queries to the challenger of consistency game of $\mdvs$. After receiving the reply $\vpk_j$ from the challenger, $\B$ forwards $\vpk_j$ %$= (\vpk_j,\vpk^{\pke})$ 
    to $\A$.
    \item $\mathcal{O}_{S}(i,S,m)$: When $\A$ makes $\mathcal{O}_{S}$ queries on $(i,S,m)$, where $S$ is the index set of the verifiers, $\B$ firstly forwards the queries to the challenger of consistency game of $\mdvs$. After receiving the response $\hat{\sigma}$ from the challenger, $\B$ encrypts the response $\hat{\sigma}$ via $\pke.\enc$ using $pk$ ($pk$ is obtained by $\pkset(\pp_{\pke},S)$), i.e., $c \leftarrow \pke.\enc(\pp_{\pke},pk,\hat{\sigma})$, and then sends the ciphertext $c$ as the signature $\sigma := c$ to $\A$.
    \item $\mathcal{O}_{V}(i,j',S,m,\sigma)$ ($j' \in S$, if $j' \notin S$, return $0$ directly): When $\A$ makes $\mathcal{O}_{V}$ queries on $(i,j',S,m,\sigma)$ where $j' \in S$, $\B$ firstly decrypts the queries $\sigma$ via $\pke.\dec$ using $sk$ (since $j' \in S$, $sk$ is obtained via $\skset(\pp_{\pke},S)$) and obtains $\hat{\sigma}$, i.e., $\hat{\sigma} \leftarrow \pke.\dec(\pp_{\pke},\vsk^{\pke},c=\sigma)$. Then, it forwards a $\mathcal{O}_{V}$ query on $(i,j',S,m,\hat{\sigma})$ to the challenger of consistency game of $\mdvs$. After receiving the bit $b$ from the challenger, $\B$ returns $b$ to $\A$.
\end{itemize}

Finally, $\A$ outputs $(i^*,S^*,m^*,\sigma^*)$. Then, $\B$ firstly decrypts the $\sigma^*$ via $\pke.\dec$ using $sk^*$ ($sk^*$ is obtained via $\skset(\pp_{\pke},S^*)$), and obtains $\hat{\sigma}^*$, i.e., $\hat{\sigma}^* \leftarrow \pke.\dec(\pp_{\pke},sk^*,c=\sigma^*)$. Then, $\B$ outputs $(i^*,S^*,m^*,\hat{\sigma}^*)$ as its final output.

That is the construction of $\B$. It is clear that $\advconspmdvs \leq \textbf{Adv}^{\textup{cons}}_{\mdvs,\B}(\lambda)$. If $\advconspmdvs$ is non-negligible, then $\textbf{Adv}^{\textup{cons}}_{\mdvs,\B}(\lambda)$ is also negligible, which is contradictory with that $\mdvs$ is a secure MDVS scheme. Thus, $\advconspmdvs$ is negligible.

\noindent \underline{\emph{Existential unforgeability.}} We assume that there exists an adversary $\A$ can win the existential unforgeability game of $\pmdvs$ with non-negligible probability. Then, we construct another adversary $\B$ to break the existential unforgeability game of $\mdvs$.

The construction is as follows.

Once $\B$ receives $\pp_{\mdvs}$ from the challenger of existential unforgeability game of $\mdvs$, $\B$ runs $\pp_{\pke} \leftarrow \pke.\setup(1^{\lambda})$ and  forwards $\pp=(\pp_{\mdvs},\pp_{\pke})$ to $\A$. 
% it  and $(\vpk^{\pke},\vsk^{\pke}) \leftarrow \pke.\kg(\pp_{\pke})$, and then sets $\pp=(\pp_{\mdvs},\pp_{\pke})$, $\vpk=(\vpk^{\mdvs},\vpk^{\pke})$. After that, it forwards $\A$ the tuple $(\pp,\spk,\vpk)$.
% $\B$ also runs $(\vpk^{\pke},\vsk^{\pke}) \leftarrow \pke.\kg(\pp_{\pke})$, such that all verifiers would get the same $(\vpk^{\pke},\vsk^{\pke})$.

Then $\B$ answers the queries from $\A$.
\begin{itemize}
    \item $\mathcal{O}_{SK}(i)$: When $\A$ makes $\mathcal{O}_{SK}$ queries on $i$, $\B$ firstly forwards the queries to the challenger of existential unforgeability game of $\mdvs$. After receiving the reply $(\spk_i,\ssk_i)$ from the challenger, $\B$ forwards $(\spk_i,\ssk_i)$ to $\A$.
    \item $\mathcal{O}_{VK}(j)$: When $\A$ makes $\mathcal{O}_{VK}$ queries on $j$, $\B$ firstly forwards the queries to the challenger of existential unforgeability game of $\mdvs$. After receiving the reply $(\vpk_j,\vsk_j)$ from the challenger, $\B$ forwards $(\vpk_j,\vsk_j)$
    % $(\vpk_j = (\vpk_j^{\mdvs},\vpk^{\pke}),\vsk_j=(\vsk_j^{\mdvs},\vsk^{\pke}))$ 
    to $\A$.
    \item $\mathcal{O}_{SPK}(i)$: When $\A$ makes $\mathcal{O}_{SPK}$ queries on $i$, $\B$ firstly forwards the queries to the challenger of existential unforgeability game of $\mdvs$. After receiving the reply $\spk_i$ from the challenger, $\B$ forwards $\spk_i$ to $\A$.
    \item $\mathcal{O}_{VPK}(j)$: When $\A$ makes $\mathcal{O}_{VPK}$ queries on $j$, $\B$ firstly forwards the queries to the challenger of existential unforgeability game of $\mdvs$. After receiving the reply $\vpk_j$ from the challenger, $\B$ forwards $\vpk_j$ 
    % $= (\vpk_j^{\mdvs},\vpk^{\pke})$ 
    to $\A$.
    \item $\mathcal{O}_{S}(i,S,m)$: When $\A$ makes $\mathcal{O}_{S}$ queries on $(i,S,m)$, where $S$ is the index set of the verifiers, $\B$ firstly forwards the queries to the challenger of existential unforgeability game of $\mdvs$. After receiving the response $\hat{\sigma}$ from the challenger, $\B$ encrypts the response $\hat{\sigma}$ via $\pke.\enc$ using $pk$ ($pk$ is obtained via $\pkset(\pp_{\pke},S)$), i.e., $c \leftarrow \pke.\enc(\pp_{\pke},pk,\hat{\sigma})$, and then sends the ciphertext $c$ as the signature $\sigma := c$ to $\A$.
    \item $\mathcal{O}_{V}(i,j',S,m,\sigma)$ ($j' \in S$, if $j' \notin S$, return $0$ directly): When $\A$ makes $\mathcal{O}_{V}$ queries on $(i,j',S,m,\sigma)$, $\B$ firstly decrypts the queries $\sigma$ via $\pke.\dec$ using $sk$ (since $j' \in S$, $sk$ is obtained via $\skset(\pp_{\pke},S)$), and obtains $\hat{\sigma}$, i.e., $\hat{\sigma} \leftarrow \pke.\dec(\pp_{\pke},sk,c=\sigma)$. Then, it forwards a $\mathcal{O}_{V}$ query on $(i,j',S,m,\hat{\sigma})$ to the challenger of existential unforgeability game of $\mdvs$. After receiving the bit $b$ from the challenger, $\B$ returns $b$ to $\A$.
\end{itemize}

Finally, $\A$ outputs $(i^*,S^*,m^*,\sigma^*)$.
%  which satisfies that: (1) for all queries $i$ to oracle $\mathcal{O}_{SK}$, it holds that $i^* \neq i$; (2) for all queries $(i,S,m)$ to oracle $\mathcal{O}_{S}$, it holds that $(i^*,S^*,m^*) \neq (i,S,m)$. 
Then, $\B$ firstly decrypts the $\sigma^*$ via $\pke.\dec$ using $sk^*$ ($sk^*$ is obtained via $\skset(\pp_{\pke},S)$), and obtains $\hat{\sigma}^*$, i.e., $\hat{\sigma}^* \leftarrow \pke.\dec(\pp_{\pke},sk^*,c=\sigma^*)$. Then, $\B$ outputs $(i^*,S^*,m^*,\hat{\sigma}^*)$ as its final output.

That is the construction of $\B$. It is clear that $\advunfpmdvs \leq \textbf{Adv}^{\textup{unf}}_{\mdvs,\B}(\lambda)$. If $\advunfpmdvs$ is non-negligible, then $\textbf{Adv}^{\textup{unf}}_{\mdvs,\B}(\lambda)$ is also negligible, which is contradictory with that $\mdvs$ is a secure MDVS scheme. Thus, $\advunfpmdvs$ is negligible.

% Once $\B$ receives $(\pp_{\mdvs},\spk,\vpk^{\mdvs})$ from the challenger of existential unforgeability game of $\mdvs$, it runs $\pp_{\pke} \leftarrow \pke.\setup(1^{\lambda})$ and $(\vpk^{\pke},\vsk^{\pke}) \leftarrow \pke.\kg(\pp_{\pke})$, and then sets $\pp=(\pp_{\mdvs},\pp_{\pke})$, $\vpk=(\vpk^{\mdvs},\vpk^{\pke})$. After that, it forwards $\A$ the tuple $(\pp,\spk,\vpk)$.

% When $\A$ makes $\mathcal{O}_{S}$ queries (i.e., querying $m$), $\B$ firstly forwards the queries to the challenger of existential unforgeability game of $\mdvs$. After receiving the response $\hat{\sigma}$ from the challenger, $\B$ encrypts the response $\hat{\sigma}$ via $\pke.\enc$ using $\vpk^{\pke}$, and then sends the ciphertext to $\A$.

% Queries (i.e., $(m,\sigma)$) to $\mathcal{O}_{V}$ are similar. $\B$ firstly decrypts the queries $\sigma$ via $\pke.\dec$ using $\vsk^{\pke}$, and obtains $\hat{\sigma}$. Then, it forwards $\mathcal{O}_{V}$ query on $(m,\hat{\sigma})$ to the challenger of existential unforgeability game of $\mdvs$. Finally, $\B$ returns what it obtains from the challenger, to $\A$.

% At last, $\A$ outputs $(m^*,\sigma^*)$ which satisfies that for all queries $m$ to $\mathcal{O}_{S}(m)$, it holds that $m^* \neq m$. Then, $\B$ firstly decrypts the queries $\sigma^*$ via $\pke.\dec$ using $\vsk^{\pke}$, and obtains $\hat{\sigma}^*$. Then, $\B$ outputs $(m,\hat{\sigma}^*)$ as its final output.

% That is the construction of $\B$. It is clear that $\advunfpdvs \leq \advunfdvs$. If $\advunfpdvs$ is non-negligible, then $\advunfdvs$ is also negligible, which is contradictory with that $\mdvs$ is a secure DVS scheme. Thus, $\advunfpdvs$ is negligible.

\noindent \underline{\emph{Pseudorandomness.}} We assume that there exists an adversary $\A$ can win the pseudorandomness game of $\pmdvs$ with non-negligible probability. Then, we construct another adversary $\B$ to break the ciphertext pseudorandomness game of $\pke$.

The construction is as follows.

Once $\B$ receives $\pp_{\pke}$ from the challenger of ciphertext pseudorandomness game of $\pke$, it runs $\pp_{\mdvs} \leftarrow \mdvs.\setup(1^{\lambda})$,
% and $(\spk,\ssk) \leftarrow \mdvs.\kg(\pp_{\pke})$, $(\vpk^{\mdvs},\vsk^{\mdvs}) \leftarrow \mdvs.\kg(\pp_{\pke})$, 
and then sets $\pp=(\pp_{\mdvs},\pp_{\pke})$.%, $\vpk=(\vpk^{\mdvs},\vpk^{\pke}=pk^{\pke})$. 
After that, it forwards $\A$ the tuple $(\pp)$.

Then $\B$ answers the queries from $\A$.

\begin{itemize}
    \item $\mathcal{O}_{SK}(i)$: When $\A$ makes $\mathcal{O}_{SK}$ queries on $i$, it proceeds as follows. If $(i,*,*,*) \in Q$, where $Q$ is the set of query-response of $\mathcal{O}_{S-chl}^{(b)}$, then it aborts. Otherwise, $\B$ runs $\mathcal{O}_{SK}(i)$ in Fig. \ref{fig:MDVS_oracle}, and obtains $(\spk_i,\ssk_i)$. After that, $\B$ forwards $(\spk_i,\ssk_i)$ to $\A$.
    \item $\mathcal{O}_{VK}(j)$: When $\A$ makes $\mathcal{O}_{VK}$ queries on $j$, $\B$ proceeds as follows. If there exists some set $S$ such that it holds $j\in S$ and $(*,S,*,*) \in Q$, where $Q$ is the set of query-response of $\mathcal{O}_{S-chl}^{(b)}$, then it aborts. Otherwise, $\B$ firstly runs $\mathcal{O}_{VK}(j)$ in Fig. \ref{fig:MDVS_oracle}, and obtains $(\vpk_j,\vsk_j)$. After that, $\B$ forwards $(\vpk_j,\vsk_j)$ 
    % $(\vpk_j = (\vpk_j^{\mdvs},\vpk^{\pke}),\vsk_j=(\vsk_j^{\mdvs},\vsk^{\pke}))$ 
    to $\A$.
    \item When $\A$ makes $\mathcal{O}_{SPK}$ queries on $i$, $\B$ runs $\spk_i \leftarrow \mathcal{O}_{SPK}(i)$ in Fig. \ref{fig:MDVS_oracle}, and returns $\spk_i$. 
    % After that, $\B$ forwards $\spk_i$ to $\A$.
    \item When $\A$ makes $\mathcal{O}_{VPK}$ queries on $j$, $\B$ firstly runs $\vpk_j \leftarrow \mathcal{O}_{VPK}(j)$ in Fig. \ref{fig:MDVS_oracle}, and returns $\vpk_j$. 
    % After that, $\B$ forwards $\vpk_j = (\spk_j^{\mdvs},\vpk^{\pke})$ to $\A$.
    \item  When $\A$ makes $\mathcal{O}_{S-chl}^{(b)}$ queries on $(i,S,m)$, where $S$ is the indices of the verifiers, $\B$ proceeds as follows. If $i$ has been queried to $\mathcal{O}_{SK}$ or there is some $j \in S$ such that $j$ has been queried to $\mathcal{O}_{VK}$, then it aborts. Otherwise, $\B$ firstly runs $\hat{\sigma} \leftarrow \mdvs.\sign(\pp_{\mdvs},\ssk_i,(\vpk_j)_{j\in S},m)$. After that, $\B$ encodes $S$ as a index $i_{S}$ (maybe via some deterministic encoding, such as a hash function or just the binary encoding), and then $\B$ forwards the $\mathcal{O}_{\enc-\textsf{Chl}}^{(b)}$ query on $(i_S, \hat{\sigma})$ to the challenger of ciphertext pseudorandomness game of $\pke$. After receiving the response $c$ from the challenger, $\B$ sends the ciphertext as the final signature $\sigma := c$ to $\A$.
    \item When $\A$ makes $\mathcal{O}_{V}$ queries on $(i,j',S,m,\sigma)$ ($j' \in S$, if $j' \notin S$, return $0$ directly), $\B$ proceeds as follows. If $(i,S,m,*) \in Q$, 
    % has been queried to the oracle $\mathcal{O}_{S}$ and the oracle outputs $\sigma$, 
    it aborts. Otherwise, $\B$ encodes $S$ as a index $i_{S}$ and forwards a $\mathcal{O}_{\dec}$ query on $(i_S,\sigma)$ to the challenger of ciphertext pseudorandomness game of $\pke$. After receiving the response $\hat{\sigma}$ from the challenger, $\B$ invokes the verification of $\mdvs$ to verify whether $\hat{\sigma}$ is a valid signature for the message $m$, i.e., $b \leftarrow \mdvs.\verify(\pp_{\mdvs},\spk_i,\vsk_{j'},(\vpk_j)_{j\in S},m,\hat{\sigma})$. Finally, $\B$ forwards $b$ to $\A$.
\end{itemize}


% When $\A$ makes $\mathcal{O}_{S-\textsf{Chl}}^{(b)}$ queries (i.e., $m$), $\B$ firstly signs the message $m$ via $\mdvs.\sign$ using $\ssk$, and obtains $\hat{\sigma}$. After that, $\B$ forwards the $\mathcal{O}_{\enc-\textsf{Chl}}^{(b)}$ query on $\hat{\sigma}$ to the challenger of pseudorandomness game of $\pke$. After receiving the response $c$ from the challenger, $\B$ sends the ciphertext as the final signature $\sigma := c$ to $\A$.

% Queries $(m,\sigma)$ to $\mathcal{O}_{V}$ are similar. $\B$ forwards a $\mathcal{O}_{\dec}$ query on $\sigma$ to the challenger of pseudorandomness game of $\pke$. After receiving the response $\hat{\sigma}$ from the challenger, $\B$ calls the verification of $\mdvs$ to verify whether $\hat{\sigma}$ is a valid signature for the message $m$. If yes, $\B$ returns $1$ to $\A$, otherwise $0$. 

Finally, $\A$ outputs a bit $b'$. Then, $\B$ outputs the bit $b'$ as its final output.

% Once $\B$ receives $(\pp_{\pke},pk^{\pke})$ from the challenger of ciphertext pseudorandomness game of $\pke$, it runs $\pp_{\mdvs} \leftarrow \mdvs.\setup(1^{\lambda})$ and $(\spk,\ssk) \leftarrow \mdvs.\kg(\pp_{\pke})$, $(\vpk^{\mdvs},\vsk^{\mdvs}) \leftarrow \mdvs.\kg(\pp_{\pke})$, and then sets $\pp=(\pp_{\mdvs},\pp_{\pke})$, $\vpk=(\vpk^{\mdvs},\vpk^{\pke}=pk^{\pke})$. After that, it forwards $\A$ the tuple $(\pp,\spk,\vpk)$.

% When $\A$ makes $\mathcal{O}_{S-\textsf{Chl}}^{(b)}$ queries (i.e., $m$), $\B$ firstly signs the message $m$ via $\mdvs.\sign$ using $\ssk$, and obtains $\hat{\sigma}$. After that, $\B$ forwards the $\mathcal{O}_{\enc-\textsf{Chl}}^{(b)}$ query on $\hat{\sigma}$ to the challenger of pseudorandomness game of $\pke$. After receiving the response $c$ from the challenger, $\B$ sends the ciphertext as the final signature $\sigma := c$ to $\A$.

% Queries $(m,\sigma)$ to $\mathcal{O}_{V}$ are similar. $\B$ forwards a $\mathcal{O}_{\dec}$ query on $\sigma$ to the challenger of pseudorandomness game of $\pke$. After receiving the response $\hat{\sigma}$ from the challenger, $\B$ calls the verification of $\mdvs$ to verify whether $\hat{\sigma}$ is a valid signature for the message $m$. If yes, $\B$ returns $1$ to $\A$, otherwise $0$. 

% At last, $\A$ outputs a bit $b$. Then, $\B$ outputs the bit $b$ as its final output.

That is the construction of $\B$. It is clear that $\advpseudopmdvs \leq \textbf{Adv}^{\textup{ct-pr}}_{\pke,\B}(\lambda)$. If $\advpseudopmdvs$ is non-negligible, then $\textbf{Adv}^{\textup{ct-pr}}_{\pke,\B}(\lambda)$ is also negligible, which is contradictory to that $\pke$ is a secure scheme that supports ciphertext pseudorandomness. Thus, $\advunfpmdvs$ is negligible.


==> 5scheme.tex <==
% \clearpage
% \blue{1, Generic MDVS construction from $\hpskem$}

% \blue{2, generic claimable MDVS construction from $\hpskem$}

% \red{3, generic MDVS construction from $\hpskem$ for illegal-message-only}

\section{Constructions of MDVS}
\label{sec:cons_mdvs}
In this section, we present several constructions of MDVS, that satisfy different security properties. In Appendix \ref{sec:concrete_scheme}, we recall a MDVS \cite{au2014strong} based on discrete logarithm. \red{Then we analyze that it supports robustness}. In Sec. \ref{sec:mdvs_claim_otr}, we extend the MDVS \cite{au2014strong} to a claimable one. To support off-the-record for any subset, in Sec. \ref{sec:fromkem}, we propose a generic construction of MDVS from a building block called $\hpskem$, which is proposed in \cite{lai2023asymmetric} and can be constructed from some standard assumptions, e.g., DDH assumption and $k$-Linear assumption. After that, we further show how to extend the generic MDVS support off-the-record for any subset to a claimable one. \red{In Appendix \ref{sec:efficientddw}, we consider a special case of MDDW, i.e.,  when $|S|=1$, and we call it DDW. Using the same framework, it requires only a DVS. In Appendix \ref{sec:efficientddw}, we present a more efficient DVS construction.}

\subsection{A claimable MDVS based on discrete logarithm}
\label{sec:mdvs_claim_otr}

Now, let's present a claimable MDVS scheme based on discrete logarithm. %in \cite{yamashita2023designated}.

Let $\sig=(\setup,\kg,\sign,\verify)$ be a (non-ring) existentially unforgeable signature scheme against adaptive chosen message attack. Let $\rsig=(\setup,\kg,\sign,\verify)$ be a ring signature. 
We require that both signature schemes are based on discrete logarithm. \red{We also present the corresponding concrete signature schemes in Appendix \ref{sec:concrete_scheme}}
Let $\prf=(\kg,\eval)$ be a PRF.
Let $\commit=(\setup,\Com,\open)$ be a commitment scheme. Then the claimable MDVS $\mdvs=(\setup,\kg,\sign,\verify,$ $\forge,\cla,\claver)$ is shown in Fig. \ref{fig:algo_cmdvs}.

% When the ring signature $\rsig$ and the non-ring signature scheme $\sig$ are based on discrete logarithm (DL), we construct a claimable MDVS (CMDVS) as shown in Fig. \ref{fig:algo_cmdvs}.

\begin{figure*}[!h]
    % \scriptsize
    \small
    % \vspace{-12pt}
    \hspace{-0.15\textwidth}
%	\centering
	%\begin{tabular}[c]{|p{18cm}|}\hline
		\fbox{
			\begin{minipage}
				% [h][5.2cm]
				[t]{0.65\textwidth}{
				\underline{$\setup(1^{\lambda})$}:\\
                $\pp_{\rsig} \leftarrow \rsig.\setup(1^{\lambda})$\\
                $\pp_{\sig} \leftarrow \sig.\setup(1^{\lambda})$\\
                $\pp_{\commit} \leftarrow \commit.\setup(1^{\lambda})$\\
                Return $\pp=(\pp_{\rsig},\pp_{\sig},\pp_{\commit})$\\

                \underline{$\kg(\pp)$}:\\
                $k \leftarrow \prf.\kg(1^{\lambda})$\\
                $(\sgsk,\sgpk) \leftarrow \sig.\kg(\pp_{\sig})$\\
                $(\rssk,\rspk) \leftarrow \rsig.\kg(\pp_{\rsig})$\\
                Return $(sk=(k,\sgsk,\rspk),pk=(\sgpk,\rspk))$\\

                \underline{$\sign(\pp,m,\sks,\Sett=(\pkvi)_{i\in[n]})$}:\\
                For each $i\in [n]$:\\
                $~~~~$$h_i := \hashf(\pks,(\pkvi)_{i\in[n]},m,i)$\\
                $~~~~$$h'_i := \hashf(\pks,(\pkvi)_{i\in[n]},m,i,1)$\\
                $\pkv=(\sgpkv=\prod_{i=1}^n \sgpkvi^{h_i},\rspkv=\prod_{i=1}^n \rspkvi^{h'_i})$\\
                % $\pkv=(\sgpkv=\prod_{i=1}^n \sgpkvi,\rspkv=\prod_{i=1}^n \rspkvi):=1$\\
                    % For $i$\\in [n]$: \\
                    % $~~~~$$h_i := \hashf(\pks,(\pkvi)_{i\in[n]},m,i)$\\
                    % $~~~~$$Y=Y\cdot \pkvi^{h_i}\
                $\sigma_{\rsig} \leftarrow \rsig.\sign(\pp_{\rsig},\rssks,(\rspks,\rspkv),m)$\\
                $r_{\sig} \leftarrow \prf.\eval(\ks,(\pks,\sigma_{\rsig},0))$\\
                $\sigma_{\sig} \leftarrow \sig.\sign(\pp_{\sig},\sgsks,(\pks,\sigma_{\rsig});r_{\sig})$\\
                $r_{\commit} \leftarrow \prf.\eval(\ks,(\pks,\sigma_{\rsig},1))$\\
                $\com \leftarrow \commit.\Com(\pp_{\commit},(\pks,\sigma_{\sig});r_{\commit})$\\
                Return $\sigma = (\sigma_{\rsig},\com)$\\

                % \underline{$\vkg(\pp)$}:\\
			 	% 	$(\skvi,\pkvi) \leftarrow \chameleon.\kg(\pp_{\cha})$\\
                %     Return $(\skvi,\pkvi)$
                \underline{$\verify(\pp,m,\pks,\sigma,\Sett)$}:\\
                For each $i\in [n]$:\\
                $~~~~$$h_i := \hashf(\pks,(\pkvi)_{i\in[n]},m,i)$\\
                $~~~~$$h'_i := \hashf(\pks,(\pkvi)_{i\in[n]},m,i,1)$\\
                $\pkv=(\sgpkv=\prod_{i=1}^n \sgpkvi^{h_i},\rspkv=\prod_{i=1}^n \rspkvi^{h'_i})$\\
                $b\leftarrow \rsig.\verify(\pp_{\rsig},(\rspks,\rspkv),m,\sigma_{\rsig})$\\
                    Return $b$
			 	}
			 \end{minipage}
			%	\vrule
			 \hspace{0.01\textwidth}
			 \begin{minipage}
			% 	% [h][5.2cm]
				[t]{0.64\textwidth}{   
                    \underline{$\forge(\pp,\pks,(\skvi)_{i\in[n]},m)$}:\\
                    For each $i\in [n]$:\\
                    $~~~~$$h_i := \hashf(\pks,(\pkvi)_{i\in[n]},m,i)$\\
                    $~~~~$$h'_i := \hashf(\pks,(\pkvi)_{i\in[n]},m,i,1)$\\
                    $\pkv=(\sgpkv=\prod_{i=1}^n \sgpkvi^{h_i},\rspkv=\prod_{i=1}^n \rspkvi^{h'_i})$\\
                    $\kv=\sum_{i=1}^n \kvi$, $\sgskv=\sum_{i=1}^n ()\sgskvi\cdot h_i$\\
                    $\rsskv=\sum_{i=1}^n (\rsskvi \cdot h'_i)$, $\skv=(\kv,\sgskv,\rsskv)$\\
                    $\sigma_{\rsig} \leftarrow \rsig.\sign(\pp_{\rsig},\rsskv,(\rspks,\rspkv),m)$\\
                    $r_{\sig} \leftarrow \prf.\eval(\kv,(\pks,\sigma_{\rsig},0))$\\
                    $\sigma_{\sig} \leftarrow \sig.\sign(\pp_{\sig},\sgskv,(\pks,\sigma_{\rsig});r_{\sig})$\\
                    $r_{\commit} \leftarrow \prf.\eval(\kv,(\pks,\sigma_{\rsig},1))$\\
                    $\com \leftarrow \commit.\Com(\pp_{\commit},(\pks,\sigma_{\sig});r_{\commit})$\\
                    Return $\sigma = (\sigma_{\rsig},\com)$\\

                    \underline{$\cla(\pp,\sks,\Sett,\sigma)$}:\\
                    % For each $i\in [n]$:\\
                    % $~~~~$$h_i := \hashf(\pks,(\pkvi)_{i\in[n]},m,i)$\\
                    % $~~~~$$h'_i := \hashf(\pks,(\pkvi)_{i\in[n]},m,i,1)$\\
                    % $\pkv=(\sgpkv=\prod_{i=1}^n \sgpkvi^{h_i},\rspkv=\prod_{i=1}^n \rspkvi^{h'_i})$\\
                    $r_{\sig} \leftarrow \prf.\eval(\ks,(\pks,\sigma_{\rsig},0))$\\
                    $r_{\commit} \leftarrow \prf.\eval(\ks,(\pks,\sigma_{\rsig},1))$\\
                    $\sigma_{\sig} \leftarrow \sig.\sign(\pp_{\sig},\sgsks,(\pks,\sigma_{\rsig});r_{\sig})$\\
                    If $\com \neq \commit.\Com(\pp_{\commit},(\pks,\sigma_{\sig});r_{\commit})$:\\
                    $~~~~$Return $\perp$\\
                    Else Return $\pi=(r_{\commit},\sigma_{\sig})$\\
                    
                    \underline{$\claver(\pp,\pks,\pkv,\sigma,\pi)$}:\\
                    If $\com \neq \commit.\Com(\pp_{\commit},(\pks,\sigma_{\sig});r_{\commit})$:\\
                    $~~~~$Return $0$\\
                    Return $b = \sig.\verify(\pp_{\sig},\sgpks,(\pks,\sigma_{\rsig}),\sigma_{\sig})$
			 	}
			 \end{minipage}	
}	
	% \setlength{\abovecaptionskip}{2pt}
	% \setlength{\belowcaptionskip}{-12pt}
	\captionsetup{justification=centering}
	\caption{Algorithms for DL based claimable multi-designated verifiers signature $\cmdvs$}
	\label{fig:algo_cmdvs}
\end{figure*}

\subsection{Generic construction of MDVS supporting off-the-record for any subset from $\hpskem$}
\label{sec:fromkem}
In this section, we provide a framework of constructing  CMDVS from $\hpskem$, and show that it achieves the required securities. 


 Let $\kemsigma=(\textsf{\upshape{KEMSetup}}, \kg, \checkkey, \encapc,\encapk,$ $ \encapc^*,\decap,\checkct)$ be a $\hpskem$  scheme supporting   universality, unexplainability,   indistinguishability, SK-second-preimage resistance and smoothness, where $\mathcal{RS}$ denotes the randomness space of $\encapc$ and $\encapk$, $\mathcal{RS}^*$ denotes the randomness space of $\encapc^*$, and $\mathcal{K}$ denotes the encapsulated key space. 

Let $\pke=(\setup,\kg,\enc,\dec)$ be an IND secure public key encryption scheme.

\red{We assume that the identity space of signers and verifiers are different. In other words, we assume that we can trivially to distinguish an identity of a signer from an identity of a verifier.} 

The CMDVS scheme $\cmdvs=(\setup,\skg,\vkg,\sign,$ $\verify,\forge)$ from $\hpskem$,   is described as follows. 

$\setup$, $\skg$ and $\vkg$ are shown in Fig. \ref{fig:new_pri_setup}, where $\setup$ directly invokes the setup algorithm of $\kemsigma$ and $\pke$. The $\skg$ invokes the key generation algorithm of $\kemsigma$ and $\pke$, while $\vkg$ only invoke the key generation algorithm of $\kemsigma$. 

\begin{figure}[!h]
	%\scriptsize
	%\hspace{-3.4cm}
	% \vspace{-12pt}
	\centering
	\small
	%\footnotesize
	%\scriptsize
	%\tiny
	\fbox{
	\begin{minipage}
% 			[h][2.8cm]
			[t]{0.7\textwidth}{
%
%Setup
%
\underline{$\textsf{Setup}(1^\lambda)$:}\\
$(\pp_{\kem},\msk)\leftarrow \kemsigma.\textsf{\upshape{KEMSetup}}(1^{\lambda})$\\
$(\pp_{\pke},\msk_{\pke}) \leftarrow \pke.\setup(1^{\lambda})$\\ 
\textup{Return} $(\pp,=(\pp_{\kem},\pp_{\pke}),\msk=(\msk_{\kem},\msk_{\pke}))$\\

%
%KG_J
%
\noindent \underline{$\skg(\pp,\msk)$:}\\ 
$(pk_{\kem},sk_{\kem}) \leftarrow \kemsigma.\kg(\pp_{\kem},\msk)$\\
$(pk_{\pke},sk_{\pke}) \leftarrow \pke.\kg(\pp_{\kem},\red{\msk_{\pke}})$\\ 
\textup{Return} $(pk=(pk_{\kem},pk_{\pke}),sk=(sk_{\kem},sk_{\pke}))$\\

\noindent \underline{$\vkg(\pp,\msk)$:}\\ 
$(pk, sk)\leftarrow \kemsigma.\kg(\pp,\msk)$\\ 
\textup{Return} $(pk, sk)$
}
	\end{minipage}
    }
%    \setlength{\abovecaptionskip}{2pt}
%	\setlength{\belowcaptionskip}{-12pt}
	\captionsetup{justification=centering}
	\caption{Algorithm descriptions of $\setup$, $\skg$ and $\vkg$}
	\label{fig:new_pri_setup}	
\end{figure}

The main body of $\cmdvs$ (i.e., $\sign$, $\verify$, $\forge$, $\claimalg$ and $\claimver$) is shown in Fig. \ref{fig:new_pri_vd}. Specifically, algorithm 
$\sign$  calls   $\encapc$ of $\kemsigma$ to generate a well-formed ciphertext with some randomness $r$, and then calls $\encapk$ with the same randomness $r$ to generate the encapsulated keys for receivers. After that, the algorithm invokes the PKE to encrypt the randomness $r$, obtaining a ciphertext $\ct$. 
Besides, it calls a NIZK proof algorithms $\textsf{NIZK}^{\R}.\textsf{PoK}$ to generate a NIZK proof, where the relation $\R$ is defined in Eq. (\ref{eq:new_ragmf}) and  $\textsf{NIZK}^{\R}=(\textsf{PoK},\textsf{PoKVer})$ is a NIZK proof using the Fiat-Shamir transform from the  Sigma protocols induced by $\kemsigma$ and $\pke$. 
% The detailed construction of \textsf{NIZK} will be postponed  in Sec. \ref{sec:nizkproof}.
The verification algorithm $\verify$ firstly calls $\textsf{NIZK}^{\R}.\textsf{PoKVer}$ to check if the NIZK proof is valid, and then calls $\decap$ with the verifier's   secret key (i.e., $\vsk_j$) to check whether the decapsulated key belongs to encapsulated key given in the signature. 
The $\forge$ algorithm firstly calls $\encapc^*$ of $\kemsigma$ with some randomness $r^*$ to generate an ill-formed ciphertext. Then, 
for each one of the verifiers  whose secret key is  not compromised, randomly samples an encapsulated key from $\mathcal{K}$; for each one of the verifiers  whose secret key is compromised, employ $\decap$ with input the corresponding secret key of the receiver,  to generate an encapsulated  key.  
After that, the algorithm invoke the PKE to encrypt the randomness $r^*$, obtain a ciphertext $\ct$.
Finally, the algorithm  calls $\textsf{NIZK}^{\R}.\textsf{PoK}$ to generate a NIZK proof.

To achieve the functionality of claimability, there are two algorithms: $\claimalg$ and $\claimver$. Both $\claimalg$ and $\claimver$ would firstly check if the NIZK proof is valid or not. The algorithm $\claimalg$ decrypts the ciphertext $\ct$ to obtain the randomness $r$, and outputs it as the proof $\pi_r$. The verification algorithm of the claimability $\claimver$ takes $\pi_r$ as input. Then, it checks if the ciphertext and the encapsulated keys are generated with the randomness $\pi_r$. If true, the algorithm outputs $1$, otherwise $0$.  

\begin{figure}[!h]
	%\scriptsize
	%\hspace{-3.4cm}
% 	\vspace{-12pt}
	\centering
	\small
	%\footnotesize
	%\scriptsize
	%\tiny
	\fbox{  %\shortstack[l]{
        \begin{minipage}
% 			[h][7.8cm]
			[t]{0.85\textwidth}{
%
%Frank
%
\underline{$\sign(\pp,\ssk_i,\{\vpk_j\}_{j\in S},m)$:}\\
$r \leftarrow \kemsigma.\RS$; $\ec \leftarrow \kemsigma.\encapc(\pp_{\kem};r)$\\
\textup{For} $ j \in S$: $\ekr \leftarrow \kemsigma.\encapk(\ppkem,\vpk_j;r)$\\%$(\ecr,\ekr) \leftarrow \encap(\pkri;\rr)$\\
%$~~~~\varepsilon_{\textup{id}'} \leftarrow e(\textsf{H}_1({\textup{id}'} ),h)^s$;
% $tag_{i}=\Htwo(\ekr)$\\
%$\alpha \leftarrow \mathbb{Z}_p^*$;  $e_{\textup{J}}=e(g,g)^{\alpha}$;
%$a_{\textup{J}}=(pk_{\textup{J}})^{\alpha}$;
%$\overline{m}=m\|\{tag_{i}\}_{\pkri \in S}$\\
$r_{\pke} \leftarrow \pke.\RS$, $\ct \leftarrow \pke.\enc(\pppke,\spk_{\pke,i},r;r_{\pke})$\\
$x \leftarrow (\ssk_{\kem,i},r,\perp,r_{\pke})$;
$y \leftarrow (\yinput)$\\
%$\overline{m}\leftarrow(m||\{\ekr\}_{\pkri \in S})$; 
$\pi \leftarrow \nizk^{\R}.\textsf{PoK}(m,x,y)$\\
\textup{Return} $\sigma \leftarrow (\alloutput)$\\%,\{tag_{i}\}_{\pkri \in S})$ \\

%\rule{14.3cm}{0.05em}
%
%Verify
%
\noindent \underline{$\verify(\pp,\spk_i,\vsk_{j'},\{\vpk_j\}_{j \in S},m,\sigma)$:}\\
%                $(hp,h,h') \leftarrow pp$; 
                $(\alloutput
%                ,\{tag_{i}\}%_{\text{id}'\in S}
				) \leftarrow \sigma$; 
                $y \leftarrow (\yinput)$\\
%             $\overline{m}\leftarrow(m||\{\ekr\}_{\pkri \in S})$\\
                \textup{If} {$\nizk^{\R}.\textsf{PoKVer}(m,\pi,y)=0$}: \textup{Return} $0$ \\
                % 	\textup{For} every $(\ec,\ek)$ in $\{\ecr,\ekr\}$:\\
                \textup{If} $ \decap(\ppkem,\vsk_{j'},\ec) \in \{\ekr\}_{j \in S} $: \textup{Return} 1\\%;
%                $\varepsilon \leftarrow e(h_{\textup{id}_{\textup{rec}}}, \varepsilon_1)(\varepsilon_2)^{r_{\textup{id}_{\textup{rec}}}} $; 
%                $tag=\Htwo(\ek)$\\
%                If $tag \not \in \{tag_{\text{id}'}\}$: \textup{Return} 0\\
                \textup{Return} $0$\\
           
           %
%RForge
%
\noindent \underline{$\forge(\pp,\spk_i,\{\vpk_j\}_{j \in S},\{\vsk_k\}_{k\in \scor},m)$:}\\
%                $\sslash S_{\text{cor}}$ here is the set of corrupted verifiers\\
				 $r^* \leftarrow \RS^*$; $\ec \leftarrow \kemsigma.\encapc^*(pp;r^*)$\\
				%  $\rr^* \leftarrow \Z$; $\ecr \leftarrow \encapc^*(pp;\rr^*)$\\
                \textup{For} $j \in S \backslash S_{\textup{cor}}$: $\ekr \leftarrow \EK$\\
                \textup{For} $k \in S_{\text{cor}}$: %\\
                % 	$~~~~$$\rr \leftarrow \Z$; 
                	$\ek_k \leftarrow \kemsigma.\decap(\ppkem,\vsk_k,\ec)$\\
				$r_{\pke} \leftarrow \pke.\RS$, $\ct \leftarrow \pke.\enc(\pppke,\spk_{\pke,i},r;r_{\pke})$\\
                $x \leftarrow (\perp,\perp,r^*,r_{\pke})$;
                $y \leftarrow (\yinput)$\\%;
%                $\overline{m}\leftarrow(m||\{\ekr\}_{\pkri \in S})$\\
                $\pi \leftarrow \nizk^{\R}.\textsf{PoK}(m,x,y)$ \\
                \textup{Return} $\sigma \leftarrow (\alloutput)$\\
				
\noindent \underline{$\claimalg(\pp,\ssk_i,\{\vpk_j\}_{j \in S},\sigma)$}\\
%                $(hp,h,h') \leftarrow pp$; 
$(\alloutput
%                ,\{tag_{i}\}%_{\text{id}'\in S}
				) \leftarrow \sigma$; 
                $y \leftarrow (\yinput)$\\
%             $\overline{m}\leftarrow(m||\{\ekr\}_{\pkri \in S})$\\
                \textup{If} {$\nizk^{\R}.\textsf{PoKVer}(m,\pi,y)=0$}: \textup{Return} $\perp$ \\
			$(\ssk_{\kem},\ssk_{\pke}) \leftarrow \ssk_i$\\
			Return $\pi_r \leftarrow \pke.\dec(\pppke,\ssk_{\pke},\ct)$\\

\noindent \underline{$\claimver(\pp,\spk_i,\{\vpk_j\}_{j\in S},\sigma,\pi_r)$}\\
%                $(hp,h,h') \leftarrow pp$; 
$(\alloutput
%                ,\{tag_{i}\}%_{\text{id}'\in S}
				) \leftarrow \sigma$; 
                $y \leftarrow (\yinput)$\\
%             $\overline{m}\leftarrow(m||\{\ekr\}_{\pkri \in S})$\\
                \textup{If} {$\nizk^{\R}.\textsf{PoKVer}(m,\pi,y)=0$}: \textup{Return} $0$ \\
				\textup{If} $c \neq \kemsigma.\encapc(\ppkem;\pi_r)$: Return $0$\\
				\textup{If} $\exists j \in S$ s.t. $\ekr \neq \kemsigma.\encapk(\ppkem,\vpk_j;\pi_r)$: Return $0$\\
				Return $1$
    }
        \end{minipage}
    }
%    \setlength{\abovecaptionskip}{2pt}
%	\setlength{\belowcaptionskip}{-12pt}
	\captionsetup{justification=centering}
	\caption{Algorithm descriptions of $\textsf{Frank}$, $\textsf{Verify}$, $\textsf{Forge}$, $\claimalg$ and $\claimver$}
	\label{fig:new_pri_vd}	
\end{figure}
    



For the NIZK proof system $\nizk^{\R}=(\textsf{PoK},\textsf{PoKVer})$ used in  Fig. \ref{fig:new_pri_vd},
% and Fig. \ref{fig:new_pri_rjf}, 
 we obtain it as follows. 
% 
% In this subsection, we show how to construct \textsf{NIZK}. 
%We first show the construction of relation $\R$ in Eq. (\ref{eq:new_ragmf}).
% to guarantee some important security features that an AGMF needs. The relation $\R$ is shown in Eq. (\ref{eq:rtilde}).
The relation $\R$ is defined in Eq. (\ref{eq:new_ragmf}).
\begin{equation}
\begin{aligned}
	\R = \{~(~&(\ssk_i,r,r^*,r_{\pke}%,
% 	\{
% 	\rr^*
	)
% 	\}_{\pkri \in S})
	,(\yinput)~): \\
	&~~~~(~(\ssk_i,\spk_i)\in \Rs\land
	(\land_{j \in S} (r,(\ec,\ekr,\vpk_j)) \in \Rck )\\
	&~~~~~~~~~\land ((r,r_{\pke}),\ct) \in \R_{\pke}~)\\
% 	\blue{(((\rj,\ecj) \in \Rc) \land ( (\rj,(\pkj,\ekj)) \in \Rk))~)}\\
% 	((\rj,(\ecj,\ekj,\pkj))\in \Rj)~) \\
	&~~~~\lor~(~(r^*,\ec)\in\Rc^*
% 	\land(\rr^*,
% % 	(
% 	\ecr
% % 	,\ekr)
% 	) \in
% 	\Rcr
% 	\Rr^*
% 	)_{\pkri \in S}
	~\land ((r^*,r_{\pke}),\ct) \in \R_{\pke})~\}
\end{aligned}
\label{eq:new_ragmf}
%\setlength{\abovedisplayskip}{3pt}
%\setlength{\belowdisplayskip}{3pt}
\end{equation}
where $\Rs$, $\Rck$ and $\Rc^*$ are defined in Eq. (\ref{eq:kemrelation}), and $\R_{\pke}$ is defiend in Eq. \eqref{eq:pkerelation}.
% where $S$ is the verifier set.%, $\R_s$ is a relation to prove knowing the sender's secret key, $(\Rj, \Rj^*)$ and $(\Rr,\Rr^*)$ are the relations as shown in Eq. (\ref{eq:relation}) for the judge and the verifiers respectively. 
Note that for every sub-relation (i.e., $\Rs$, $\Rck$, $\Rc^*$ and $\R_{\pke}$), the $\hpskem$ and PKE guarantees that there is a Sigma protocol. So, with the technique of trivially combining Sigma protocols for AND/OR proofs  \cite[Sec. 19.7]{BS20}, we obtain a new Sigma protocol for relation $\R$. Then, using the Fiat-Shamir transform, we derive a NIZK proof system $\nizk^{\R}=(\textsf{PoK},\textsf{PoKVer})$ for $\R$ in the random oracle model.% then using the composition operations of Sigma protocol, e.g. ``AND/OR'' operation of Sigma protocols \cite[Sec. 19.7]{BS20} with Fiat-Shamir heuristic \cite{FS86}, the composited NIZK proof also works well.

% % =======explanation of relation $\R$==============
Now, we provide some explanations about relation $\R$.

The first part (i.e., $((\ssk_i,\spk_i)\in \Rs \land
	(\land_{j \in S} (r,(\ec,\ekr,\vpk_j)) \in \Rck ) \land ((r,r_{\pke}),\ct) \in \R_{\pke})$ ) of the expression of $\R$ contains three sub-parts: (i) $((\ssk_i,\spk_i)\in \Rs)$ guarantees  the authentication of the signer; (ii) $(\land_{j \in S} (r,(\ec,\ekr,\vpk_j)) \in \Rck )$ guarantees that the ciphertext $\ec$ and the corresponding encapsulated key $\ekr$ for the verifiers are well-formed,
and further  convinces the verifier that all verifiers would accept $\ec$ and   $\ekr$ (i.e., satisfying consistency); (iii) $((r,r_{\pke}),\ct) \in \R_{\pke}$ guarantees that the plaintext with respect to $\ct$ is the randomness to generate $\ec$ and $\ekr$.

The second part (i.e., $((r^*,\ec)\in \Rc^* \land ((r^*,r_{\pke}),\ct) \in \R_{\pke})$) of the expression of  $\R$ is prepared  to guarantee the property of off-the-record (i.e., deniability). More specifically, it is prepared for the forgers (including the universal and/or the verifiers) to construct a valid NIZK proof, since they do not know the signer's secret key. The forging algorithm in Fig. \ref{fig:new_pri_vd} shows that the forgers can generate the ill-formed ciphertext via $\encapc^*(\pp;r^*)$. 
Therefore, the forgers can always obtain the witness $r^*$ for the second part of $\R$. In addition, $((r^*,r_{\pke}),\ct) \in \R_{\pke}$ guarantees that the plaintext of with respect to $\ct$ the randomness to generate the ill-formed ciphertext $\ec$.

The relation $\R$ combines the two parts with an ``OR'' operation, so either the signer or the forgers can generate a valid NIZK proof for  $\R$.

%\begin{remark}
%In our framework $\mdvs$, in order to reduce the size of signature, all $\ekr$ are all encapsulated in the same ciphertext $c$. This suggests that $\kgj$ and $\kgu$ are built based  on the identical  $\hpskem$. Actually, $\ekj$ can be encapsulated in another  ciphertext, which can be generated with an independent $\hpskem$. Hence, the judge can run $\kgj$ based on  an independent $\hpskem$, to generate the  public/secret key pair. In this case, the obtained AGMF  can support third-party moderation better.
%
%%the ciphertext and the encapsulated key for the judge are also  generated based on a 
%
%
%
%% During the generation of AGMF signature, $\ekj$ and $\ekr$ are all encapsulated in the same ciphertext $c$. 
%
%% In other words, 
%
%% the judge and the user share the same $c$
%
%% In our framework $\AGMF$, the moderator and the users share the same parameter to generate public/secret key pairs, 
%
%% which suggests that the moderator and the users are in the same system. 
%\end{remark}

% $((\rr',\ec) \in\R_1^*)$ indicates that the ciphertext $\ecr$ is generated by $\encap_1^*$, which means that calling $\decap$, the verifier accept the signature with negligible probability.


\vspace{1mm}
\noindent \textbf{Correctness.} Now we show the correctness of the above scheme $\cmdvs$ here. % The correctness requires that $\textsf{Verify}$ and $\textsf{Judge}$ both return $1$ when receiving a valid AGMF signature. 
For any signer $i$, any message $m \in \M$, any verifier identity sets $S$ and any $\mu \in S$,
when given public parameters and  master secret key
$(\pp,\msk)\leftarrow \setup(1^{\lambda})$,  given signer's key pair $
            (\spk_i,\ssk_i) \leftarrow \skg(\pp,\msk)$,  given verifiers' key pairs $( (\vpk_j,\vsk_j) \leftarrow \skg(\pp,\msk))_{j \in S}$, and given a signature $
            \sigma \leftarrow \sign(\pp,$ $\ssk_i,\{\vpk_j\}_{j \in S}, m)$,    
%$\sigma \leftarrow \sign(pp,\sks,S,\pkj,m)$ and any  $\pkr \in S$, 
we first parse  $\sigma=(\alloutput) $, and let $y :=(\yinput)$. %and  $\overline{m}:=(m||\{\ekr\}_{\pkri \in S})$. 

We analyze the output  of $\textsf{Verify}$ as follows: (i) the correctness of $\nizk^{\R}$  guarantees that $\textsf{NIZK}^{\R}.\textsf{PoKVer}(m,\pi,y)=1$; (ii) the correctness of $\kemsigma$ guarantees that $\decap(\pp,\vsk_{\mu},\ec)\in \{\ekr\}_{j \in S}$ when $c=\encap(\pp;r)$, $\ekr=\encapk(\pp,\vpk_j;r)$ for each $j\in S$, and $\mu \in S$. So, $\textsf{Verify}$ will return $1$, which implies that the above $\cmdvs$ is correct. 

\red{claimability}

\vspace{1.5mm}

\noindent \textbf{Security. } 
For security, we have the following theorem.

%For accountability, we have the following two theorems. The proofs are presented in Appendix \ref{appendix:r-bind} and Appendix \ref{appendix:s-bind}.

\begin{theorem}\label{thm:security}
	If a $\hpskem$  scheme $\kemsigma$ is \red{universal, unexplainable, indistinguishble, SK-second-preimage resistant and smooth}, \red{a $\pke$ scheme is IND secure}, and  $\nizk^{\R}=(\textsf{\upshape{PoK}},$ $\textsf{\upshape{PoKVer}})$ is a Fiat-Shamir NIZK proof system for $\mathcal{R}$, then  our scheme $\cmdvs$ is consistent, existential unforgeable, off-the-record, and has privacy of designated verifiers identities.
\end{theorem}

We put the proof of Theorem \ref{thm:security}  in Appendix \ref{sec:appendix_proof_of_mdvs}. 
% the proof of Theorem \ref{thm:security} will be given in the appendixes.
Specifically, the proof of consistency is in Appendix \ref{sec:proof_cons}.
The proof of existential unforgeability is presented in 
 Appendix \ref{sec:proof_unf}.
For the property of off-the-record, the proofs are in Appendix \ref{sec:proof_otr}.
The proof of PVI is given in Appendix \ref{sec:proof_pvi}. 





==> 8discussion.tex <==
\section{Discussion}
Other topic:\\
%set constrained encryption\\
%deniability or off-the-record\\
%Claimable, using \cite{yamashita2023designated}\\
If the underlying (M)DVS itself supports pseudorandomness, then the framework doesn't require the XOR computation (i.e., codes in Line \ref{code:markone} and \ref{code:marktwo} of Algorithm \ref{alg:Watmtwo}, and codes in Line \ref{code:markthree} of Algorithm \ref{alg:Dettwotwo}), which would be easier. For your interest, we can provide pseudorandom DVS in Appendix \red{xxx}. However, we do not provide pseudorandom MDVS. We left it as an open problem. \\
error-correcting code

==> DDW_construction.tex <==
\section{DDW construction}\label{sec:ddw_construction}

\subsection{Generic construction}\label{sec:ddw_generic_construction}

Let  $\dvs=(\dvs.\setup,\skg,\vkg,\sign,\verify)$ be a DVS scheme with signature length  $\lambda_{\sigma}$. Let $\M$ denote  the message space of $\dvs$. Let \red{$H_1:\{0,1\}^*\rightarrow\M$} and  $H_2:\{0,1\}^*\rightarrow\{0,1\}$ be two hash functions, both of which will be modeled as  random oracles in the security proof. 

Our DDW scheme $\ddw_{n,\ell,\lambda_{\sigma}}=(\setup,\wkg,\dkg,\watm,$ $\detect)$, for some predefined parameters $n$ and $\ell$, is as follows.\footnote{Note that according to Assumption \ref{assumption},  any contiguous block of $\ell$ tokens contains at least $\alpha$ bits of min-entropy.}
\begin{myitemize}
	\item
	$\setup(1^\lambda)$: Compute $\pp\leftarrow \dvs.\setup(1^\lambda)$, and return $\pp$ as the public parameter  of DDW. 
	\item
	$\wkg(\pp)$: Generate  $(\spk,\ssk)\leftarrow\skg(\pp)$, and set $\wpk=\spk$ and $\wsk=\ssk$. Return $(\wpk,\wsk)$. 
	\item
	$\dkg(\pp)$: Generate  $(\vpk,\vsk)\leftarrow\vkg(\pp)$, and set $\dpk=\vpk$ and $\dsk=\vsk$. Return $(\dpk,\dsk)$. 
	\item $\watm(\pp,\wsk,\dpk,\bm{\rho})$: Its description is shown in \textbf{Algorithm \ref{alg:DDW_Watm}}.
	\item $\detect(\pp,\wpk,\dsk,\bm{t})$: Its description is shown in \textbf{Algorithm \ref{alg:DDW_Det}}. 
\end{myitemize}


\begin{algorithm}
	\caption{$\watm(\pp,\wsk,\dpk,\bm{\rho})$ \label{alg:DDW_Watm} }
	$\ssk\leftarrow \wsk$, 	
	~$~\vpk\leftarrow\dpk$
	
	$\bm{t}\leftarrow\epsilon$
	
	\While{$|\bm{t}|+\ell+\lambda_{\sigma}<n$}{
		$\bm{t}\leftarrow\bm{t}||\genmodel_\ell(\bm{\rho},\bm{t})$
		
		$\bm{\sigma}\leftarrow\sign(\pp,\ssk,\vpk, \red{H_1}(\bm{t}[-\ell]))$
		
		$\bm{\sigma}_{\textup{prev}}\leftarrow\epsilon$, $~\bm{m}\leftarrow\epsilon$
		
		\While{$\bm{\sigma}\neq\epsilon$}{
			$\sigma\leftarrow \bm{\sigma}[0]$, $~\bm{\sigma}\leftarrow\bm{\sigma}[1:]$
			
			$\bm{x}\leftarrow\genmodel_\ell(\bm{\rho},\bm{t})$
			
			\While{$H_2(\bm{m}||\bm{x}||\bm{\sigma}_{\textup{prev}})\neq\sigma$}{
				$\bm{x}\leftarrow\genmodel_\ell(\bm{\rho},\bm{t})$}
			$\bm{m}\leftarrow\bm{m}||\bm{x}$, $~\bm{t}\leftarrow\bm{t}||\bm{x}$, $~\bm{\sigma}_{\textup{prev}}\leftarrow\bm{\sigma}_{\textup{prev}}||\sigma$
		}
	}
	\If{$|\bm{t}|<n$}{
		$\bm{t}\leftarrow\bm{t}||\genmodel_{n-|\bm{t}|}(\bm{\rho},\bm{t})$
	}
	
	\Return $\bm{t}$
\end{algorithm}

\begin{algorithm}
	\caption{$\detect(\pp,\wpk,\dsk,\bm{t})$ \label{alg:DDW_Det} }
	$\spk\leftarrow \wpk$, 	
	$~\vsk\leftarrow\dsk$
	
	\For{$i\in[n-(\ell+\lambda_{\sigma})]$}{
		$\widetilde{m}\leftarrow H_1(\bm{t}[i:i+\ell])$
				
		$\bm{\sigma}\leftarrow\epsilon$, 		
		$~\bm{m}\leftarrow\epsilon$
		
		\For{$j\in[\lambda_{\sigma}]$}{
			$\bm{m}\leftarrow\bm{m}||\bm{t}[i+j\cdot\ell+1:i+j\cdot\ell+\ell]$
			
			$\bm{\sigma}\leftarrow\bm{\sigma}||H_2(\bm{m}||\bm{\sigma})$
		}
		\If{$\verify(\pp,\spk,\vsk,\widetilde{m},\bm{\sigma})=1$}{\Return 1}
	}
	\Return 0
	
\end{algorithm}

\subsection{Security proofs}\label{sec:ddw_security_proof}
Now, we show that our proposed $\ddw$ satisfies completeness, soundness,  distortion-freeness and robustness.

\begin{theorem}[Completeness]\label{thm:ddw_complete}
	$\ddw$ is  $\ell$-complete. 
\end{theorem}
\begin{proof}
	For any normally generated $\pp$, $(\wpk,\wsk)$ and $(\dpk,\dsk)$, any prompt $\bm{\rho}\in\mathcal{T}^*$, and  any token $\widehat{\bm{t}}\leftarrow\watm(\pp,\wsk,\dpk,\bm{\rho})$, if   $\watm$  successfully embeds in a message/signature pair in $\widehat{\bm{t}}$, obviously the correctness of the underlying DVS scheme guarantees that  $\detect(\pp,\wpk,\dsk,\widehat{\bm{t}})=1$. The only possibility that $\watm$ fails in embedding  is that  the rejection sampling algorithm 	fails to find the next batch of tokens whose hash is consistent with the target bit (i.e., line 10-12 in Algorithm \ref{alg:DDW_Watm}). Note that by Assumption \ref{assumption}, any $\ell$ consecutive tokens generated by $\genmodel_{\ell}$  contains $\alpha$ bits of entropy. So no one can predict the input to the random oracle in line 10  of Algorithm \ref{alg:DDW_Watm} except with probability $2^{-\alpha}$, which is negligible. In other words, with overwhelming probability, the random oracle in line 10  of Algorithm \ref{alg:DDW_Watm} will return a uniformly and independently sampled bit. 
	Hence, with overwhelming probability, we derive that for each sampling attempt  of the next batch of tokens, it will succeed in finding a consistent hash value  with probability $\frac{1}{2}$.  After $\textsf{poly}(\lambda)$ 	attempts, the rejection sampling will find the next batch of tokens with probability $1-2^{-\lambda}$, i.e., the probability that $\watm$ fails is negligible. 
\end{proof}

\begin{theorem}[Soundness]\label{thm:ddw_sound}
	$\ddw$ is $\ell$-sound. 
\end{theorem}
\begin{proof}
	%If there exists a PPT adversary $\A$ that can find a text labeled as watermarked, it must mean that this
	%watermarked text has a valid message/signature pair embedded inside. Then, one may extract this pair, which constitutes a forgery attack against the underlying signature scheme \qed
	
	For any PPT adversary $\A$ attacking the soundness of $\ddw$, we show a PPT adversary $\B$ attacking the existential unforgeability of the underlying $\dvs$ as follows. 
	
	Upon receiving $(\pp,\spk,\vpk)$, $\B$ sets $\wpk=\spk$ and $\dpk=\vpk$, and 
	sends $(\pp,\wpk,\dpk)$ to $\A$. %	the public parameter $\pp$ (note that the public parameter $\pp$ generated by $\setup$ of $\ddw$ is the same as that generated by the underlying $\dvs.\setup$), $\B$ sends $\pp$ to $\A$. 
	$\B$ maintains two local arrays, $L_{\text{ro},1}$ and  $L_{\text{ro},2}$, to keep track of $\A$'s random oracle queries. Then, $\B$  answers $\A$'s oracle queries as below: 
	\begin{myitemize}
		\item \underline{$\mathcal{O}_{RO,1}(str)$:} If there is some $(str,y)\in L_{\text{ro}}$,  $\mathcal{B}$ returns $y$; otherwise,  $\mathcal{B}$  samples $y\leftarrow\M$, adds $(str,y)$ to $L_{\text{ro},1}$, and returns $y$. 
		
		\item \underline{$\mathcal{O}_{RO,2}(str)$:} If there is some $(str,y)\in L_{\text{ro}}$,  $\mathcal{B}$ returns $y$; otherwise,  $\mathcal{B}$  samples $y\leftarrow\{0,1\}$, adds $(str,y)$ to $L_{\text{ro},2}$, and returns $y$. 
				
		\item\underline{$\mathcal{O}_{W}(\bm{\rho})$:}  $\B$ runs algorithm $\textsf{SimWatMar}$ (with the help of its  signing oracle $\mathcal{O}_S$)   as shown in  Algorithm \ref{alg:DDW_SimWatm}. More specifically, Algorithm \ref{alg:DDW_SimWatm} is the same as Algorithm \ref{alg:DDW_Watm}, except that   the original  hash functions $H_1$ and $H_2$ (in line 5 and line 10, respectively) in  Algorithm \ref{alg:DDW_Watm} are replaced with random oracles, and the original $\sign$ algorithm  (in line 5) in  Algorithm \ref{alg:DDW_Watm} is replaced with $\B$'s signing oracle $\mathcal{O}_S$. Finally, $\B$ 
		returns the output $\bm{t}$ of $\textsf{SimWatMar}$  to $\A$.
		
		%    	\item\underline{$\mathcal{O}_{W}(i,S,\bm{\rho})$:}  $\B$ firstly queries its own oracle $\mathcal{O}_{SK}(i)$ to obtain $(\spk_i,\ssk_i)$, and sets $(\wpk_i,\wsk_i)=(\spk_i,\ssk_i)$. Then,  for all $j\in S$, it queries its own oracle $\mathcal{O}_{VPK}(j)$ to obtain $\vpk_j$ and sets $\dpk_j=\vpk_j$.  Subsequently,  it runs algorithm $\watm$ with input $(\pp,\wsk_i,(\dpk_j)_{j\in S},\bm{\rho})$ as shown in  Algorithm \ref{alg:Watm}, with the exceptions  that:
		%    \begin{itemize}
			%    	\item It uses random oracle to replace the hash function $H$ in  Algorithm \ref{alg:Watm}. Specifically, when computing the hash function $H(\bm{t}[-\ell])$ in line 6 (in  Algorithm \ref{alg:Watm}), it obtains $y$ via querying $\mathcal{O}_{RO}(\bm{t}[-\ell])$, and sets $y=H(\bm{t}[-\ell])$; when   computing the hash function $H(\bm{m}||\bm{x}||\bm{\sigma}_{\text{prev}})$ in line 12 (in  Algorithm \ref{alg:Watm}), it obtains $y$ querying $\mathcal{O}_{RO}(\bm{m}||\bm{x}||\bm{\sigma}_{\text{prev}})$, and sets $y=H(\bm{m}||\bm{x}||\bm{\sigma}_{\text{prev}})$. 
			%    	\item It uses its own oracle $\mathcal{O}_{S}$ to replace algorithm $\mdvs.\sign$ in  Algorithm \ref{alg:Watm}.  Specifically, when computing $\mdvs.\sign(\pp,\ssk_i,(\vpk_j)_{j\in S}, H(\bm{t}[-\ell]))$ in line  6 (in  Algorithm \ref{alg:Watm}), it queries its own oracle $\mathcal{O}_S(i,S,H(\bm{t}[-\ell]))$ to obtain $\sigma'$, and sets $\mdvs.\sign(\pp,\ssk_i,(\vpk_j)_{j\in S}, H(\bm{t}[-\ell]))=\sigma'$ (i.e., $\bm{\sigma}=\sigma'$ in line 6). 
			%    \end{itemize} 
		%    Finally, $\B$ returns the output $\bm{t}$ of $\watm$ (with the above modifications) to $\A$.
		
		\item\underline{$\mathcal{O}_{D}(\bm{t})$:}  $\B$  runs algorithm $\textsf{SimDetect}$ (with the help of its verification oracle $\mathcal{O}_V$) as shown in  Algorithm \ref{alg:DDW_SimDet}. More specifically, Algorithm \ref{alg:DDW_SimDet} is the same as Algorithm \ref{alg:DDW_Det}, except that   the original  hash functions $H_1$ and $H_2$ (in line 3 and line 7, respectively) in  Algorithm \ref{alg:DDW_Det} are  replaced with  random oracles, and the original $\verify$ (in line 9) in  Algorithm \ref{alg:DDW_Det} is replaced with $\B$'s verification oracle $\mathcal{O}_V$. 
		Finally, $\B$ returns the output of $\textsf{SimDetect}$  to $\A$. 
		
		%    	\item\underline{$\mathcal{O}_{D}(i,j',S,\bm{t})$:}  $\B$ firstly queries its own oracle $\mathcal{O}_{SPK}(i)$ (resp., $\mathcal{O}_{VK}(j')$) to obtain $\spk_i$ (resp., $(\vpk_{j'},\vsk_{j'})$), and sets $\wpk_i=\spk_i$ (resp., $(\dpk_{j'},\dsk_{j'})=(\vpk_{j'},\vsk_{j'})$). Then, for all $j\in S$, it queries its own oracle $\mathcal{O}_{VPK}(j)$ to obtain $\vpk_j$ and sets $\dpk_j=\vpk_j$.  Subsequently,  it runs algorithm $\detect$ with input $(\pp,\wpk_i,\dsk_{j'},(\dpk_j)_{j\in S},\bm{t})$ as shown in  Algorithm \ref{alg:Det}, with the exceptions  that:
		%    \begin{itemize}
			%    	\item It uses random oracle to replace the hash function $H$ in  Algorithm \ref{alg:Det}. Specifically, when computing the hash function $H(\bm{t}[i:i+\ell])$ in line 4 (in  Algorithm \ref{alg:Det}), it obtains $y$ via querying $\mathcal{O}_{RO}(\bm{t}[i:i+\ell])$, and sets $y=H(\bm{t}[i:i+\ell])$; when   computing the hash function $H(\bm{m}||\bm{\sigma})$ in line 9 (in  Algorithm \ref{alg:Det}), it obtains $y$ querying $\mathcal{O}_{RO}(\bm{m}||\bm{\sigma})$, and sets $y=H(\bm{m}||\bm{\sigma})$. 
			%    	\item It uses its own oracle $\mathcal{O}_{V}$ to replace algorithm $\mdvs.\verify$ in  Algorithm \ref{alg:Det}.  Specifically, when computing $\mdvs.\verify(\pp,\spk_i,\vsk_{j'},\red{(\vpk_j)_{j\in S},} \bm{m},\bm{\sigma})$ in line  11 (in  Algorithm \ref{alg:Det}), it queries its own oracle $\mathcal{O}_V(i,j',S,m=\bm{m}, \sigma=\bm{\sigma})$ to obtain $b$, and sets $\mdvs.\verify(\pp,\spk_i,\vsk_{j'},\red{(\vpk_j)_{j\in S},} \bm{m},\bm{\sigma})=b$  in line 11. 
			%    \end{itemize} 
		%    Finally, $\B$ returns the output of $\detect$ (with the above modifications) to $\A$. 
	\end{myitemize}
	
	Receiving $\bm{t}^*$ from $\A$, $\B$  checks whether  $\textsf{SimDetect}(\pp,\wpk,\bm{t}^*)=1$ or not (with the help of its verification oracle $\mathcal{O}_V$). 
	\begin{myitemize}
		\item[-] If so, $\B$ extracts $(\widetilde{m},\bm{\sigma})$ according to the steps in Algorithm \ref{alg:DDW_SimDet} (from line 1 to line 8), and sets $(\widehat{m^*},\widehat{\sigma^*})=(\widetilde{m},\bm{\sigma})$. 
		\item[-] Otherwise, $\B$ uniformly samples  $(\widehat{m^*},\widehat{\sigma^*})$ from the message space and the signature space. 
	\end{myitemize} 
	Finally, $\B$ returns $(\widehat{m^*},\widehat{\sigma^*})$ as its final output. 
	
	\begin{algorithm}
		\caption{$\textsf{SimWatMar}^{\mathcal{O}_S,\mathcal{O}_{RO,1},\mathcal{O}_{RO,2}}(\pp,\dpk,\bm{\rho})$ \label{alg:DDW_SimWatm}}
	%	$\ssk_i\leftarrow \wsk_i$
		
		$\vpk\leftarrow\dpk$
		
		$\bm{t}\leftarrow\epsilon$
		
		\While{$|\bm{t}|+\ell+\lambda_{\sigma}<n$}{
			$\bm{t}\leftarrow\bm{t}||\genmodel_\ell(\bm{\rho},\bm{t})$
			
			$\bm{\sigma}\leftarrow\underline{\mathcal{O}_{S}(\underline{\mathcal{O}_{RO,1}}(\bm{t}[-\ell]))}$
			
			$\bm{\sigma}_{\textup{prev}}\leftarrow\varepsilon$, 			
			$~\bm{m}\leftarrow\epsilon$
			
			\While{$\bm{\sigma}\neq\epsilon$}{
					$\sigma\leftarrow \bm{\sigma}[0]$, $~\bm{\sigma}\leftarrow\bm{\sigma}[1:]$
				
				$\bm{x}\leftarrow\genmodel_\ell(\bm{\rho},\bm{t})$
				
				\While{$\underline{\mathcal{O}_{RO,2}}(\bm{m}||\bm{x}||\bm{\sigma}_{\textup{prev}})\neq\sigma$}{
					$\bm{x}\leftarrow\genmodel_\ell(\bm{\rho},\bm{t})$}
				$\bm{m}\leftarrow\bm{m}||\bm{x}$, 		
				$~\bm{t}\leftarrow\bm{t}||\bm{x}$, 		
				$~\bm{\sigma}_{\textup{prev}}\leftarrow\bm{\sigma}_{\textup{prev}}||\sigma$
			}
		}
		\If{$|\bm{t}|<n$}{
			$\bm{t}\leftarrow\bm{t}||\genmodel_{n-|\bm{t}|}(\bm{\rho},\bm{t})$
		}
		
		\Return $\bm{t}$
	\end{algorithm}
	
	\begin{algorithm}
		\caption{$\textsf{SimDetect}^{\mathcal{O}_{V},\mathcal{O}_{RO,1},\mathcal{O}_{RO,2}}(\pp,\wpk,\bm{t})$ \label{alg:DDW_SimDet}}
		$\spk\leftarrow \wpk$
		
		\For{$i\in[n-(\ell+\lambda_{\sigma})]$}{
			$\widetilde{m}\leftarrow \underline{\mathcal{O}_{RO,1}}(\bm{t}[i:i+\ell])$
			
			$\bm{\sigma}\leftarrow\epsilon$, 			
			$~\bm{m}\leftarrow\epsilon$
			
			\For{$j\in[\lambda_{\sigma}]$}{
				$\bm{m}\leftarrow\bm{m}||\bm{t}[i+j\cdot\ell+1:i+j\cdot\ell+\ell]$
				
				$\bm{\sigma}\leftarrow\bm{\sigma}||\underline{\mathcal{O}_{RO,2}}(\bm{m}||\bm{\sigma})$
			}
			\If{$\underline{\mathcal{O}_V(\widetilde{m},\bm{\sigma})}=1$}{\Return 1}
		}
		\Return 0
		
	\end{algorithm}
	
	
	That is the construction of adversary $\B$. Now we turn to analyze its advantage. 
	
	It is easy to see that $\B$ perfectly simulates game  $\gamesoundddw$ for $\A$. Note that when $\A$ wins  $\gamesoundddw$, $\A$'s final output $\bm{t}^*$ satisfies $(\detect(\pp,\wpk,\dsk,\bm{t}^*)=1)\wedge(\textsf{nonoverlap}_{\ell}(\bm{t}^*,\bm{t}_1,\bm{t}_2,\cdots)=1)$, where $\bm{t}_1,\bm{t}_2,\cdots$ are the watermarked texts that $\A$ receives via querying $\orawatm$. 	
	The fact  $\detect(\pp,\wpk,\dsk,\bm{t}^*)=1$ implies that there must be some $i'\in[n-(\ell+\lambda_{\sigma})]$, such that for $\widetilde{m}=\mathcal{O}_{RO,1}(\bm{t}^*[i':i'+\ell])$ and for $\bm{\sigma}$ generated according to line 4-8 in Algorithm \ref{alg:DDW_Det} (when $i=i'$), $\verify(\pp,\spk,\vsk,\widetilde{m},\bm{\sigma})=1$. On the other hand, $\textsf{nonoverlap}_{\ell}(\bm{t}^*,\bm{t}_1,$ $\bm{t}_2,\cdots)=1$ guarantees that during the process of answering $\A$'s $\mathcal{O}_W$-oracle queries,  the random oracle $\mathcal{O}_{RO,1}$ has never been programmed on $\bm{t}^*[i':i'+\ell]$.  So the property of random oracle guarantees that $\widetilde{m}=\mathcal{O}_{RO,1}(\bm{t}^*[i':i'+\ell])$ has never been submitted as a signing query by $\B$. 
	
	Hence, $\B$ wins   $\textup{\textbf{G}}^{\textup{eunf}}_{\dvs,\B}(\lambda)$  if  $\A$ wins  $\gamesoundddw$, i.e., 
	\begin{eqnarray*}
		\textup{\textbf{Adv}}^{\textup{eunf}}_{\dvs,\B}(\lambda)\geq \advsoundddw,
	\end{eqnarray*}
	concluding the proof of this theorem. 
\end{proof}
\begin{remark}
\red{We stress that if the underlying DVS scheme meets strong unforgeability, $\ddw$ achieves $(\lambda_{\sigma}+1)\ell$-soundness.}
\end{remark}

\begin{theorem}[Distortion-freeness]\label{thm:ddw_distor-free}
	$\ddw$ is $k$-distortion-free. 
\end{theorem}
\begin{proof}
	We show the proof with a sequence of games. 
	
	\noindent\textbf{Game} $\textbf{G}_0$: This game is the original $\gamedistorddw$ when $b$ is fixed to be $0$. Note that in this game, when $\A$ queries the oracle $\mathcal{O}^{(0)}_{M\text{-}chl}$ on $\bm{\rho}$, the challenger runs Algorithm \ref{alg:DDW_Watm} with input $(\pp,\wsk,\dpk,\bm{\rho})$ and returns the output to $\A$.
	
	\noindent\textbf{Game} $\textbf{G}_1$: This game is the same as  $\textbf{G}_0$, except that when $\A$ queries the oracle $\mathcal{O}^{(0)}_{M\text{-}chl}$ on $\bm{\rho}$, the challenger runs Algorithm \ref{alg:DDW_Watm} with the following modifications: in line 5 of Algorithm \ref{alg:DDW_Watm}, $\bm{\sigma}$ is uniformly sampled from the DVS signature space.
	
	\noindent\textbf{Game} $\textbf{G}_2$: This game is the original $\gamedistorddw$ when $b$ is fixed to be $1$.
	
	We present the following two lemmas with postponed proofs.
	\begin{lemma}\label{lem:DDW_distor_1}
		$|\Pr[\mathbf{G}_1=1]-\Pr[\mathbf{G}_0=1]|\leq 2\textup{\textbf{Adv}}^{\textup{ps-rand}}_{\dvs,\A'}(\lambda)$ for some PPT adversary $\A'$.
	\end{lemma}
	\begin{lemma}\label{lem:DDW_distor_2}
		\red{$|\Pr[\mathbf{G}_2=1]-\Pr[\mathbf{G}_1=1]|\leq 2^{-\alpha}$.}
	\end{lemma}
	
	Combining these two lemmas, we derive that for any PPT adversary $\A$, 
	\begin{eqnarray*}
		\advdistorddw\leq \textup{\textbf{Adv}}^{\textup{ps-rand}}_{\dvs,\A'}(\lambda)+2^{-\alpha-1}.
	\end{eqnarray*}
	
	Hence, what remains is to prove the above two lemmas.
	\begin{proof}[Proof of Lemma \ref{lem:DDW_distor_1}]
		We show a PPT adversary $\A'$   attacking the  pseudorandomness of the underlying  $\dvs$ as follows. 
		
		Upon receiving $\pp$ (note that the public parameter  $\pp$ generated by $\setup$ of $\ddw$ is the same as that generated by the underlying $\dvs.\setup$), $\A'$ sends $\pp$ to $\A$. $\A'$ maintains a local array $L_{\text{ro}}$ to keep track of $\A$'s random oracle queries (we use $\mathcal{Y}$ to denote the range of the hash function modelled as a random oracle). Then, $\A'$  answers $\A$'s oracle queries as below: 
		\begin{myitemize}
			\item \underline{$\mathcal{O}_{RO}(str)$:} If there is some $(str,y)\in L_{\text{ro}}$,  $\A'$ returns $y$; otherwise,  $\A'$  samples $y\leftarrow\mathcal{Y}$, adds $(str,y)$ to $L_{\text{ro}}$, and returns $y$. 
			
			\item\underline{$\mathcal{O}_{\textsf{Model}}(\bm{\rho})$:} $\A'$ returns $\textsf{Model}(\bm{\rho})$ to $\A$. 
			
			\item\underline{$\mathcal{O}_{M\text{-}chl}^{(0)}(\bm{\rho})$:}  $\A'$  runs algorithm $\watm$ on input $(\pp,\wsk_i,(\dpk_j)_{j\in S},\bm{\rho})$ (as shown in  Algorithm \ref{alg:Watm}) with the exception that  in line 6 of  Algorithm \ref{alg:Watm}, $\bm{\sigma}$ is generated via querying its own oracle $\mathcal{O}_{S\text{-}chl}^{(b)}(i,S,H(\bm{t}[-\ell]))$ (i.e., ``$\bm{\sigma}\leftarrow\mdvs.\sign(\pp,\ssk_i,(\vpk_j)_{j\in S},$  $H(\bm{t}[-\ell]))$'' is replaced with ``$\bm{\sigma}\leftarrow\mathcal{O}_{S\text{-}chl}^{(b)}(i,S,H(\bm{t}[-\ell]))$''). Finally, 	  $\A'$
			returns the output $\bm{t}$ of the modified $\watm$  to $\A$.
			
			
			
			\item\underline{$\mathcal{O}_{D}(i,j',S,\bm{t})$:}  $\A'$ firstly queries its own oracle $\mathcal{O}_{SPK}(i)$ (resp., $\mathcal{O}_{VK}(j')$) to obtain $\spk_i$ (resp., $(\vpk_{j'},\vsk_{j'})$), and sets $\wpk_i=\spk_i$ (resp., $(\dpk_{j'},\dsk_{j'})=(\vpk_{j'},\vsk_{j'})$). Then, for all $j\in S$, it queries its own oracle $\mathcal{O}_{VPK}(j)$ to obtain $\vpk_j$ and sets $\dpk_j=\vpk_j$.  Subsequently,  it runs algorithm $\detect$ on input $(\pp,\wpk_i,\dsk_{j'},\red{(\dpk_j)_{j\in S}},\bm{t})$ (as shown in  Algorithm \ref{alg:Det}) with the exception that in line 11 of Algorithm \ref{alg:Det}, ``\textbf{if} $\mdvs.\verify(\pp,\spk_i,\vsk_{j'},\bm{m},\bm{\sigma})=1$'' is replaced with ``\textbf{if} $\oravk(i,j',S,\bm{m},\bm{\sigma})=1$''. 
			Finally, 	  $\A'$ returns the output of the modified  $\detect$  to $\A$. 
			
			%    	\item\underline{$\mathcal{O}_{D}(i,j',S,\bm{t})$:}  $\B$ firstly queries its own oracle $\mathcal{O}_{SPK}(i)$ (resp., $\mathcal{O}_{VK}(j')$) to obtain $\spk_i$ (resp., $(\vpk_{j'},\vsk_{j'})$), and sets $\wpk_i=\spk_i$ (resp., $(\dpk_{j'},\dsk_{j'})=(\vpk_{j'},\vsk_{j'})$). Then, for all $j\in S$, it queries its own oracle $\mathcal{O}_{VPK}(j)$ to obtain $\vpk_j$ and sets $\dpk_j=\vpk_j$.  Subsequently,  it runs algorithm $\detect$ with input $(\pp,\wpk_i,\dsk_{j'},(\dpk_j)_{j\in S},\bm{t})$ as shown in  Algorithm \ref{alg:Det}, with the exceptions  that:
			%    \begin{itemize}
				%    	\item It uses random oracle to replace the hash function $H$ in  Algorithm \ref{alg:Det}. Specifically, when computing the hash function $H(\bm{t}[i:i+\ell])$ in line 4 (in  Algorithm \ref{alg:Det}), it obtains $y$ via querying $\mathcal{O}_{RO}(\bm{t}[i:i+\ell])$, and sets $y=H(\bm{t}[i:i+\ell])$; when   computing the hash function $H(\bm{m}||\bm{\sigma})$ in line 9 (in  Algorithm \ref{alg:Det}), it obtains $y$ querying $\mathcal{O}_{RO}(\bm{m}||\bm{\sigma})$, and sets $y=H(\bm{m}||\bm{\sigma})$. 
				%    	\item It uses its own oracle $\mathcal{O}_{V}$ to replace algorithm $\mdvs.\verify$ in  Algorithm \ref{alg:Det}.  Specifically, when computing $\mdvs.\verify(\pp,\spk_i,\vsk_{j'},\red{(\vpk_j)_{j\in S},} \bm{m},\bm{\sigma})$ in line  11 (in  Algorithm \ref{alg:Det}), it queries its own oracle $\mathcal{O}_V(i,j',S,m=\bm{m}, \sigma=\bm{\sigma})$ to obtain $b$, and sets $\mdvs.\verify(\pp,\spk_i,\vsk_{j'},\red{(\vpk_j)_{j\in S},} \bm{m},\bm{\sigma})=b$  in line 11. 
				%    \end{itemize} 
			%    Finally, $\B$ returns the output of $\detect$ (with the above modifications) to $\A$. 
		\end{myitemize}
		
		Receiving $\A$'s final output $b'$, $\A'$ returns $b'$ as its own final output. 
		
		That's the construction of adversary $\A'$. 
		
		It is evident  that when the challenge bit in $\textup{\textbf{G}}^{\textup{ps-rand}}_{\mdvs,\A'}(\lambda)$ is 0 (resp., 1), $\A'$ perfectly simulates game $\textbf{G}_0$ (resp., $\textbf{G}_1$) for $\A$. \red{(need more explanation...)} 
		
		So we derive 
		\begin{eqnarray*}
			\textup{\textbf{Adv}}^{\textup{ps-rand}}_{\mdvs,\A'}(\lambda)\geq \frac{1}{2}|\Pr[\mathbf{G}_1=1]-\Pr[\mathbf{G}_0=1]|,
		\end{eqnarray*}
		concluding the proof of this theorem. 
		
		
	\end{proof}
	\begin{proof}[Proof of Lemma \ref{lem:DDW_distor_2}]
		\red{TBC}
	\end{proof}
	
	
\end{proof}


\begin{theorem}[Robustness]\label{thm:ddw_robust}
	$\ddw$ is $\delta$-robust. 
\end{theorem}
\begin{proof}
	\red{In game $\gamerobddw$, note that $\A$'s final output $\bm{t}$ satisfies that  a $\delta$-length segment of  $\bm{t}^*$ that does verify remains (i.e., a valid message/signature pair is embedded in this segment) in $\bm{t}$. 
		Hence, Algorithm \ref{alg:Det} will extract the  message/signature pair from $\bm{t}$, leading to a successful detection output.} 
	
	
	
	%	Let $\bm{t}$ denote the output of the LLM. If the adversary’s
	%	output A(t) contains 2δ consecutive tokens from the original t, it must mean that there is a δ consecutive
	%	tokens, which embeds a message/signature pair, is preserved in A(t). The detection algorithm will recover
	%	this consecutive sequence by an exhaustive search, resulting in a successful detection output
\end{proof}


==> DDW_definition.tex <==
\section{Designated detectable watermarking}\label{sec:ddw_definition}
A \emph{designated detectable watermarking (DDW)} scheme for an auto-regressive model $\model$ over token vocabulary $\tg$ is a tuple of algorithms $\ddw=(\setup,$ $\wkg,\dkg,\watm,\detect)$, where 
\begin{myitemize}
	\item
	$\setup(1^\lambda) \rightarrow \pp$: On input the security parameter $\lambda$, it outputs a  public parameter $\pp$.
	\item
	$\wkg(\pp) \rightarrow (\wpk,\wsk)$: On input $\pp$, it outputs a public/secret key pair $(\wpk,\wsk)$ for watermarking. 
	\item
	$\dkg(\pp) \rightarrow (\dpk,\dsk)$: On input  $\pp$, it outputs a public/secret key pair $(\dpk,\dsk)$ for detecting.
	\item $\watm(\pp,\wsk,\dpk,\bm{\rho}) \rightarrow \bm{t}$: On input   $\pp$, a secret watermarking key $\wsk$, a  public detecting key $\dpk$, and a prompt $\bm{\rho}\in\tg^*$, it outputs a response text  $\bm{t}\in\tg^*$.
	\item $\detect(\pp,\wpk,\dsk,\bm{t}) \rightarrow b$: On input  $\pp$, a public watermarking key $\wpk_i$, a secret detecting key $\dsk$,   and a candidate watermarked text  $\bm{t}\in\tg^*$, it outputs a bit $b$: $b = 1$ (accept) or $b = 0$ (reject).
\end{myitemize}

The DDW scheme should satisfy completeness,  soundness,  distortion-freeness, and robustness. Most of these properties are   defined with  games providing adversaries with access to the following  oracles. 
\begin{description}
	\item \textbf{Watermarking Oracle:} $\mathcal{O}_{W}(\bm{\rho})$
	\begin{enumerate}
		\item Output $\bm{t}\leftarrow \watm(\pp,\wsk,\dpk,\bm{\rho})$.
	\end{enumerate}
	
	\item \textbf{Detecting Oracle:} $\mathcal{O}_{D}(\bm{t})$
	\begin{enumerate}
		\item Output $b\leftarrow\detect(\pp,\wpk,\dsk,\bm{t})$.
	\end{enumerate}
	
\end{description}

Now we turn to the formal definitions of the required properties.

\begin{definition}{\textbf{\textup{(Completeness).}}}
	We say that $\ddw$ is \emph{$\ell$-complete}, if for  any prompt $\bm{\rho}\in\tg^*$,   it holds that
	\begin{equation*}
		\Pr \left [
		\begin{array}{l}
			\pp\leftarrow \setup(1^{\lambda}),\\
			(\wpk,\wsk)\leftarrow\wkg(\pp),\\
			(\dpk,\dsk) \leftarrow \dkg(\pp),\\
			\bm{t} \leftarrow \watm(\pp,\wsk,\dpk, \bm{\rho})\\
			~~~~\text{s.t.}~|\bm{t}|\geq \ell
		\end{array}
		~ \textup{\Large{:}}~
		\detect(\pp,\wpk,\dsk,\bm{t})\neq 1
		\right ] \leq \negl.
	\end{equation*}
	%\label{def:mddw_correct}
\end{definition}

\begin{definition}{\textbf{\textup{(Soundness).}}}
	We say that $\ddw$ is \emph{$k$-sound}, if for   any PPT adversary $\A$ and any prompt $\bm{\rho}\in\tg^*$,  %any detector set $S$ and any $j'\in S$, 
	\[\advsoundddw=\Pr[\gamesoundddw=1] \leq \negl \] 
	where $\gamesoundddw$ is shown in Fig. \ref{fig:ddw_sound}, and the predicate $\textsf{\upshape{nonoverlap}}_k$ $(\bm{t}^*,\bm{t}_1,\bm{t}_2,\cdots)$ in Fig. \ref{fig:ddw_sound} outputs 1 if  $\bm{t}^*$ does not share a $k$-length window of tokens with any of the genuinely-watermarked texts $\bm{t}_1,\bm{t}_2,\cdots$, and outputs 0 otherwise. 
\end{definition}

\begin{figure}[t!]\small
	\centering
	% \hspace{-0.06\textwidth}
	\fbox{\shortstack[l]{
			\underline{$\gamesoundddw$:}\\
			$\pp \leftarrow \setup(1^{\lambda})$, $(\wpk,\wsk)\leftarrow\wkg(\pp)$, 
			$(\dpk,\dsk) \leftarrow \dkg(\pp)$\\
			$\bm{t}^* \leftarrow \A^{\orawatm,\oradet}(\pp,\wpk,\dpk)$\\
			$\qquad$where  all  $\bm{t}_1,\bm{t}_2,\cdots$ (denoting the watermarked texts that $\A$ receives\\
			$\qquad$via querying $\orawatm$) satisfy  $\textsf{nonoverlap}_k(\bm{t}^*,\bm{t}_1,\bm{t}_2,\cdots)=1$.\\
			If 	 $\detect(\pp,\wpk,\dsk,\bm{t}^*)=1$, then return $1$,\\
			Else return $0$
		}
	}
	\captionsetup{justification=centering}
	\caption{Game for defining $k$-soundness of DDW}
	\label{fig:ddw_sound}
\end{figure}  

\begin{definition}{\textbf{\textup{(Distortion-freeness).}}}
	We say that $\ddw$ is \emph{$k$-distortion-free}, if for   any PPT adversary   $\A$,   %any detector set $S$ and any $j'\in S$, 
	\[\advdistorddw=|\Pr[\gamedistorddw=1]-\frac{1}{2}|\leq \negl \] 
	where $\gamedistorddw$ is shown in Fig. \ref{fig:ddw_distortion-free}, and the predicate $\textsf{\upshape{nonoverlap}}_k(\bm{t},\bm{t}')$ in Fig. \ref{fig:ddw_distortion-free} outputs 1 if  $\bm{t}$ does not share a $k$-length window of tokens with $\bm{t}'$, and outputs 0 otherwise. 
\end{definition}

\begin{figure}[t!]\small
	\centering
	% \hspace{-0.06\textwidth}
	\fbox{\shortstack[l]{
			\underline{$\gamedistorddw$:}\\
			$(\pp,\msk) \leftarrow \setup(1^{\lambda})$, $b\leftarrow \{0,1\}$\\ $(\wpk,\wsk)\leftarrow\wkg(\pp)$, 
			$(\dpk,\dsk) \leftarrow \dkg(\pp)$\\
			$b' \leftarrow \A^{\mathcal{O}_{\textsf{Model}},\mathcal{O}_{M\text{-}chl}^{(b)},\oradet}(\pp)$\\
			$\qquad$where $\mathcal{O}_{\textsf{Model}}(\bm{\rho})$ outputs $\textsf{Model}(\bm{\rho})$, $\mathcal{O}_{M\text{-}chl}^{(0)}(\bm{\rho})$ outputs $\orawatm(\bm{\rho})$,\\
			$\qquad$$\mathcal{O}_{M\text{-}chl}^{(1)}(\bm{\rho})$ outputs  $\genmodel(\bm{\rho})$,\\
			$\qquad$let $R$ denote the set of responses returned by   $\mathcal{O}_{M\text{-}chl}^{(b)}$,\\
%			$\qquad$all queries $(i,S,\bm{\rho})$ to   $\mathcal{O}_{M\text{-}chl}^{(b)}$ should satisfy that for all $j\in S$, $j$ has never been queried to $\oradk$,  \\ 
%			$\qquad$all queries $j$ to   $\oradk$ should satisfy that there is no  $(i,S,*,\bm{t})\in Q$ satisfying $j\in S$,  \\ 
			$\qquad$and  all queries $\bm{t}'$ to $\oradet$ should satisfy: $\forall~\bm{t}\in R$, $\textsf{nonoverlap}_k(\bm{t}',\bm{t})=1$ \\
			If $b'=b$, then return $1$,\\
			Else return $0$
	}		}
	\captionsetup{justification=centering}
	\caption{Game for defining $k$-distortion-freeness of DDW}
	\label{fig:ddw_distortion-free}
\end{figure}  

\begin{definition}{\textbf{\textup{(Robustness).}}}
	We say that $\ddw$ is \emph{$\delta$-robust}, if for   any PPT adversary   $\A$,  
	\[\advrobddw=\Pr[\gamerobddw=1] \leq \negl \] 
	where $\gamerobddw$ is shown in Fig. \ref{fig:ddw_rob} . 
	%, and the predicate $\textsf{\upshape{nonoverlap}}_k(\bm{t},\bm{t}')$ in Fig. \ref{fig:mddw_rob} outputs 1 if  $\bm{t}$ does not share a $k$-length window of tokens with $\bm{t}'$, and outputs 0 otherwise. 
\end{definition}

\begin{figure}[t!]\small
	\centering
	% \hspace{-0.06\textwidth}
	\fbox{\shortstack[l]{
			\underline{$\gamerobddw$:}\\
			$(\pp,\msk) \leftarrow \setup(1^{\lambda})$, $(\wpk,\wsk)\leftarrow\wkg(\pp)$\\
			$(\dpk,\dsk) \leftarrow \dkg(\pp)$, $\bm{t}^*\leftarrow\watm(\pp,\wsk,\dpk,\bm{\rho})$\\
			$\bm{t}\leftarrow\A^{\orawatm,\oradet}(\pp,\wpk,\dpk,\bm{t}^*)$\\
			$\qquad$where \red{a $\delta$-length segment of $\bm{t}^*$  remains in $\bm{t}$}\\
			If  $\detect(\pp,\wpk,\dsk,\bm{t})=0$, then return $1$,\\
			Else return $0$
	}		}
	\captionsetup{justification=centering}
	\caption{Game for defining $\delta$-robustness of DDW}
	\label{fig:ddw_rob}
\end{figure}  




==> DVS_definition.tex <==
\section{Designated verifier signature}
\label{sec:def_dvs}
We recall the definition of designated verifier signature (DVS) following \cite{LV04}.

Let $\mathcal{PK}_s$ be a  public  key space of signers, $\mathcal{SK}_s$ be a secret key space of signers, $\mathcal{PK}_v$ be a public  key space of verifiers, $\mathcal{SK}_v$ be a secret key space of verifiers, $\mathcal{M}$ be a message space and $\mathcal{SG}$ be a signature space. Without loss of generality, we assume that  all signers' public-key inputs are in $\mathcal{PK}_s$, all signers' secret-key inputs are in $\mathcal{SK}_s$, all verifiers' public-key inputs are in $\mathcal{PK}_v$, all verifiers' secret-key inputs are in $\mathcal{SK}_v$, all message inputs are in $\mathcal{M}$, and all signature inputs are in $\mathcal{SG}$.



A designated verifier signature scheme is a tuple of algorithms $\dvs=(\setup,$ $\skg,\vkg,\sign,\verify)$, where 
\begin{myitemize}
%\setlength{\itemindent}{0em}
	\item
	$\setup(1^\lambda) \rightarrow \pp$: On input the security parameter $\lambda$, it outputs a public parameter $\pp$.
	\item
	$\skg(\pp) \rightarrow (\spk,\ssk)$: On input  $\pp$, it outputs the public key $\spk$ and secret key $\ssk$ for a signer. 
	\item
	$\vkg(\pp) \rightarrow (\vpk,\vsk)$: On input  $\pp$, it outputs the public key $\vpk$ and secret key $\vsk$ for a verifier.
	\item $\sign(\pp,\ssk,\vpk,m) \rightarrow \sigma$: On input  $\pp$, a  signing secret  key $\ssk$, a    verifying public key $\vpk$ and a message $m$, it outputs a signature $\sigma$.
	\item $\verify(\pp,\spk,\vsk,m,\sigma) \rightarrow b$: On input   $\pp$, a  signing public  key $\spk$, a  verifying secret key $\vsk$,  a message $m$, and a signature $\sigma$, it outputs a bit $b$: $b = 1$ (accept) or $b = 0$ (reject).
\end{myitemize}
%\begin{itemize}
%	\item[\textbullet]
%	$\setup(1^\lambda) \rightarrow \pp$: On input the security parameter $\lambda$, it outputs public parameters $\pp$.
%	\item[\textbullet]
%	$\skg(\pp,\msk) \rightarrow (\spk,\ssk)$: On input  $\pp$ and  $\msk$, it outputs the public key $\spk$ and secret key $\ssk$ for a signer. 
%	\item[\textbullet]
%	$\vkg(\pp,\msk) \rightarrow (\vpk,\vsk)$: On input  $\pp$ and  $\msk$, it outputs the public key $\vpk$ and secret key $\vsk$ for a verifier.
%	\item[\textbullet] $\sign(\pp,\ssk,\vpk,m) \rightarrow \sigma$: On input  $\pp$, a  signing secret  key $\ssk$, a    verifying public key $\vpk$ and a message $m$, it outputs a signature $\sigma$.
%	\item[\textbullet] $\verify(\pp,\spk,\vsk,m,\sigma) \rightarrow b$: On input   $\pp$, a  signing public  key $\spk$, a  verifying secret key $\vsk$,  a message $m$, and a signature $\sigma$, it outputs a bit $b$: $b = 1$ (accept) or $b = 0$ (reject).
%\end{itemize}

The DVS scheme should satisfy the following properties, which are  defined with security games providing adversaries with access to the following  oracles.
\begin{description}
	\item \textbf{Signing Oracle:} $\mathcal{O}_{S}(m)$
	\begin{enumerate}
		\item Output $\sigma\leftarrow \sign(\pp,\ssk,\vpk,m)$.
	\end{enumerate}
	
	\item \textbf{Verification Oracle:} $\mathcal{O}_{V}(m,\sigma)$
	\begin{enumerate}
		\item Output $b\leftarrow\verify(\pp,\spk,\vsk,m,\sigma)$.
	\end{enumerate}
	
\end{description} 

\begin{definition}{\textbf{\textup{(Correctness).}}}
	We say that $\dvs$ is correct, if for any message $m \in \M$,  it holds that
	\begin{equation*}
		\Pr \left [
		\begin{array}{l}
			\pp\leftarrow \setup(1^{\lambda})\\
			(\spk,\ssk) \leftarrow \skg(\pp)\\
			(\vpk,\vsk) \leftarrow \vkg(\pp)\\
			\sigma \leftarrow \sign(\pp,\ssk,\vpk, m)
		\end{array}
		~ \textup{\Large{:}}~
		\verify(\pp,\spk,\vsk,m,\sigma)\neq 1
		\right ] = 0.
	\end{equation*}
	\label{def:dvs_correct}
\end{definition}

\begin{definition}{\textbf{\textup{(Existential unforgeability).}}}
	We say that $\dvs$ is existentially unforgeable, if for all PPT adversary $\A$, 
	\[\advunfdvs=\Pr[\gameunfdvs=1] \leq \negl \] where $\gameunfdvs$ defined in Fig. \ref{fig:dvs_unf}.
	\label{def:dvs_unf}
\end{definition}
\begin{figure}[t!]\small
	\centering
	% \hspace{-0.06\textwidth}
	\fbox{\shortstack[l]{
			\underline{$\gameunfdvs$:}\\
			$\pp \leftarrow \setup(1^{\lambda})$, $(\spk,\ssk) \leftarrow \skg(\pp)$, 
			$(\vpk,\vsk) \leftarrow \vkg(\pp)$\\
			$(m^*,\sigma^*) \leftarrow \A^{\orasign,\oraver}(\pp,\spk,\vpk)$\\
			$\qquad$where for all queries  $m$ to $\orasign$:  $m^* \neq m$.\\
			If $\verify(\pp,\spk,\vsk,m^*,\sigma^*)=1$, then  return $1$\\
			Else, return $0$
		}
	}
	\captionsetup{justification=centering}
	\caption{Game for defining existential unforgeability of DVS}
	\label{fig:dvs_unf}
\end{figure}  

\begin{definition}{\textbf{\textup{(Pseudorandomness).}}}
	We say that $\dvs$ is pseudorandom, if for all PPT adversary $\A$,  
	\[\advpseudodvs=|\Pr[\gamepseudodvs=1]-\frac{1}{2}| \leq \negl \] 
	where $\gamepseudodvs$ defined in Fig. \ref{fig:dvs_pseudorandom}.  
	\label{def:dvs_pseudo}
\end{definition}

\begin{figure}[t!]\small
	\centering
	% \hspace{-0.06\textwidth}
	\fbox{\shortstack[l]{
			\underline{$\gamepseudodvs$:}\\
			$\pp \leftarrow \setup(1^{\lambda})$, $b\leftarrow \{0,1\}$\\ 
			$(\spk,\ssk) \leftarrow \skg(\pp)$, 
			$(\vpk,\vsk) \leftarrow \vkg(\pp)$\\
			$b' \leftarrow \A^{\mathcal{O}_{S\text{-}chl}^{(b)},\oraver}(\pp,\spk,\vpk)$\\
			$\qquad$where  $\mathcal{O}_{S\text{-}chl}^{(0)}(m)$ outputs $\orasign(m)$,  $\mathcal{O}_{S\text{-}chl}^{(1)}(m)$ outputs a uniformly\\
				$\qquad$sampled $\sigma\leftarrow\mathcal{SG}$, 		let  $Q$ denote the set of query-response of  $\mathcal{O}_{S\text{-}chl}^{(b)}$,\\
			$\qquad$and all queries $(m',\sigma')$ to $\oraver$ should satisfy  $(m',\sigma')\notin Q$ \\
			If $b'=b$, then return $1$,\\
			Else return $0$
	}		}
	\captionsetup{justification=centering}
	\caption{Game for defining pseudorandomness of DVS}
	\label{fig:dvs_pseudorandom}
\end{figure}  

%\begin{definition}{\textbf{\textup{\red{(Privacy of signer's identity)}.}}}
%	We say that $\mdvs$ is PSI secure, if for all PPT adversary $\A$, its advantage 
%	\[\advpsidvs=|\Pr[\gamepsidvs=1]-\frac{1}{2}| \leq \negl \] 
%	where $\gamepsidvs$ defined in Fig. \ref{fig:dvs_psi}.  
%	\label{def:dvs_psi}
%\end{definition}
%
%\begin{figure}[t!]\small
%	\centering
%	% \hspace{-0.06\textwidth}
%	\fbox{\shortstack[l]{
%			\underline{$\gamepsidvs$:}\\
%			$\pp \leftarrow \setup(1^{\lambda})$, $b\leftarrow \{0,1\}$\\
%			$(\spk_0,\ssk_0) \leftarrow \skg(\pp)$, $(\spk_1,\ssk_1) \leftarrow \skg(\pp)$, 
%			$(\vpk,\vsk) \leftarrow \vkg(\pp)$\\
%			$b' \leftarrow \A^{\mathcal{O}_{S,0},\mathcal{O}_{S,1},\mathcal{O}_{S\text{-}chl}^{(b)},\oraver}(\pp,\spk_0,\spk_1,\vpk)$\\
%			$\qquad$where $\mathcal{O}_{S,0}(m)$ outputs $\sign(\pp,\ssk_0,\vpk,m)$, $\mathcal{O}_{S,1}(m)$ outputs $\sign(\pp,\ssk_1,\vpk,m)$, \\ $\qquad$$\mathcal{O}_{S\text{-}chl}^{(b)}(m)$ outputs $\sign(\pp,\ssk_b,\vpk,m)$, \\
%			$\qquad$letting $Q$ denote the set of query-response of  $\mathcal{O}_{S\text{-}chl}^{(b)}$,\\
%			$\qquad$and all queries $(m',\sigma')$ to $\oraver$ should satisfy that there is no  $(m',\sigma')\in Q$ \\
%			If $b'=b$, then return $1$,\\
%			Else return $0$
%	}		}
%	\captionsetup{justification=centering}
%	\caption{Game for defining privacy of signer's identity of DVS}
%	\label{fig:dvs_psi}
%\end{figure}  



==> PKEctpr.tex <==
\subsection{PKE with pseudorandom ciphertext}
\label{sec:pre_pke}
We firstly recall the definition of public key encryption (PKE) and its ciphertext pseudorandomness, following \cite{moller2004public}. 

\begin{definition}
    A public-key encryption scheme $\pke$ consists of four algorithms $\pke=(\setup,\kg,\enc,\dec)$:
    \begin{myitemize}
        \item $\setup(1^{\lambda}) \rightarrow \pp$: On input the security parameter, it outputs a public parameter $\pp$.
        \item $\kg(\pp) \rightarrow (pk,sk)$: On input  $\pp$, it outputs a public key $pk$ and a secret key  $sk$.
        \item $\enc(\pp,pk,m) \rightarrow c$: On input  $\pp$, the public key $pk$ and a message $m$, it outputs a ciphertext $c$.
        \item $\dec(\pp,sk,c) \rightarrow m/\bot$: On input  $\pp$, the secret key $sk$ and a ciphertext $c$, it outputs a message $m$ or a failure symbol $\bot$. 
    \end{myitemize}
\end{definition}

The correctness requires that for any valid message $m$, 
\begin{equation*}
    \Pr \left [
    \begin{array}{l}
        \pp\leftarrow \setup(1^{\lambda})\\
        (pk,sk) \leftarrow \kg(\pp)\\
        c \leftarrow \enc(\pp,pk, m)
    \end{array}
    ~ \textup{\Large{:}}~
    \dec(\pp,sk,c) = m
    \right ] \geq 1 - \negl.
\end{equation*}

% Please refer to \cite{moller2004public} 
%We omit the definitions for the security notions of IND-CPA or IND-CCA. Here, we present the security notion of ciphertext pseudorandomness.

\begin{definition} We say that $\pke$ (with ciphertext space $\mathcal{C}$) has ciphertext pseudorandomness, if for all PPT adversary $\A$,  \[\advpseudopke=|\Pr[\gamepseudopke=1]-\frac{1}{2}| \leq \negl \] 
	where $\gamepseudopke$ is defined in Fig. \ref{fig:pke_pseudorandom}. 
    
\end{definition}

\begin{figure}[!h]\small
	\centering
	% \hspace{-0.06\textwidth}
	\fbox{\parbox{\linewidth}{\shortstack[l]{
			\underline{$\gamepseudopke$:}\\
			$\pp \leftarrow \setup(1^{\lambda})$, $b\leftarrow \{0,1\}$\\
            % $(pk,sk) \leftarrow \kg(\pp)$\\
			$b' \leftarrow \A^{\mathcal{O}_{KG},\mathcal{O}_{PK},\mathcal{O}_{\enc-chl}^{(b)},\mathcal{O}_{\dec}}(\pp)$\\
			$\qquad$where  $\mathcal{O}_{\enc-chl}^{(0)}(i,m)$ outputs $\enc(\pp,pk_i,m)$ ($pk_i$ is obtained  from\\ $\qquad\qquad$$\mathcal{O}_{PK}(i)$),\\
            $\qquad$$\mathcal{O}_{\enc-chl}^{(1)}(i,m)$ outputs a uniformly sampled $c\leftarrow\mathcal{C}$,\\
          %  $\qquad$$\mathcal{O}_{\dec}(i,c)$ returns $\dec(\pp,sk_i,c)$ ($sk_i$ is output by $\mathcal{O}_{KG}$),\\
         %   $\qquad$$\mathcal{O}_{KG}(i)$ returns $(pk_i,sk_i) \leftarrow \kg(\pp)$ for the first call on $i$,\\
       %     $\qquad\qquad$and simply output $(pk_i,sk_i)$ for subsequent call,\\
            $\qquad$$\mathcal{O}_{PK}(i)$ returns a public key $pk_i$ output by $\mathcal{O}_{KG}(i)$ for $i$,\\
            $\qquad$let $Q$ denote the set of query-response of $\mathcal{O}^{(b)}_{\enc-chl}$,\\  
			$\qquad$all queries $i$ to $\mathcal{O}_{KG}$ should satisfy $(i,*) \notin Q$,\\
            $\qquad$and all queries $(i,c)$ to $\mathcal{O}_{\dec}$ should satisfy  $(i,c)\notin Q$ \\
			If $b'=b$, then return $1$\\
			Else return $0$
	}		}}
	\fbox{\parbox{\linewidth}{
		\textbf{Key Generation Oracle} $\mathcal{O}_{KG}(i)$:
		\begin{enumerate}
			\item On the first call to $\mathcal{O}_{KG}$ on  $i$, compute $(pk_i,sk_i)\leftarrow\kg(\pp)$, output and store $(pk_i,sk_i)$.
			\item On subsequent calls, simply output $(pk_i,sk_i)$. 
		\end{enumerate}
		\vspace{0.4\baselineskip}
		\textbf{Public Key Generation Oracle}  $\mathcal{O}_{PK}(i)$: 
		\begin{enumerate}
			\item $(pk_i,sk_i)\leftarrow\mathcal{O}_{KG}(i)$; output  $pk_i$.
		\end{enumerate}
	\vspace{0.4\baselineskip}
	\textbf{Decryption Oracle} $\mathcal{O}_{\dec}(i,c)$: 
	\begin{enumerate}
		\item $(pk_i,sk_i)\leftarrow\mathcal{O}_{KG}(i)$; output  $\dec(\pp,sk_i,c)$.
	\end{enumerate}
}		}
	\captionsetup{justification=centering}
	\caption{Game $\gamepseudopke$ for PKE}
	\label{fig:pke_pseudorandom}
\end{figure}  

==> ToDoList.tex <==
\section{\red{To-do list}}

\begin{enumerate}
\item Add the descriptions of three distinct entities in Sec. \ref{sec:language_model}.

%\item Add more details about generic construction of MDDW in Sec. \ref{sec:generic_construction}.

\item Add theorem and security proof in Sec. \ref{sec:security_proof}.

%\item Add definition of pseudorandomness of MDVS (Definition \ref{def:mdvs_pseudo}).

%\item Check the description of generative models.

\item Check the oracles which are actually needed, which can be removed.  

\item Add the concrete construction of MDVS, and check whether $(\vpk_j)_{j\in S}$ are needed in the  $\verify$ algorithm for construction.

\item Analyze the parameters.

\end{enumerate}

--------------------------------------
